Estimating the Impact of BGP Prefix Hijacking

BGP prefix hijacking is a critical threat to the resilience and security of communications in the Internet. While several mechanisms have been proposed to prevent, detect or mitigate hijacking events, it has not been studied how to accurately quantify the impact of an ongoing hijack. When detecting a hijack, existing methods do not estimate how many networks in the Internet are affected (before and/or after its mitigation). In this paper, we study fundamental and practical aspects of the problem of estimating the impact of an ongoing hijack through network measurements. We derive analytical results for the involved trade-offs and limits, and investigate the performance of different measurement approaches (control/data-plane measurements) and use of public measurement infrastructure. Our findings provide useful insights for the design of accurate hijack impact estimation methodologies. Based on these insights, we design (i) a lightweight and practical estimation methodology that employs ping measurements, and (ii) an estimator that employs public infrastructure measurements and eliminates correlations between them to improve the accuracy. We validate the proposed methodologies and findings against results from hijacking experiments we conduct in the real Internet.

==> ML_estimator.tex <==



The methodology we propose uses information (i) provided by RC monitors about the AS-paths to the victim and hijacker ASes, and (ii) about AS routing policies, to adapt the estimations of NIE-RC towards more accurate estimations \vkotronis{The latter needs some rephrasing I think}. It is summarized as follows:

\begin{tcolorbox}
\textbf{LRE-RC: Hijack impact estimation from route collectors measurements.}
\begin{enumerate}[leftmargin=*]
\item Collect the AS-paths seen from the $M$ RC monitors for prefixes of the victim ($IP_{V}$) and hijacker ($IP_{H}$) ASes before the hijack, and for the hijacked prefix after the hijack ($IP_{*}$).
\item Calculate the NIE seen by RC monitors for $IP_{*}$
\item Calculate one of the following quantities/features:

\begin{enumerate}
\item Calculate the fraction of the RC monitors that have a shorter paths to $IP_{V}$ than to $IP_{H}$ (and vice-versa). Specifically, for each monitor $i\in\mathcal{M}$, calculate the length of its paths to $IP_{V}$ ($dist\_V_{i}$) and to $IP_{H}$ ($dist\_H_{i}$), and calculate the quantity 
\begin{equation*}
f_{dist} = \frac{1}{M}\sum_{i\in\mathcal{M}}\mathbb{I}_{dist\_V_{i}<dist\_H_{i}}-\mathbb{I}_{dist\_H_{i}<dist\_V_{i}}
\end{equation*}
where $\mathbb{I}$ the indicator function ($\mathbb{I}_{x}=1$ if $x$ is true and $\mathbb{I}_{x}=0$ otherwise)

\item Calculate the fraction of the RC monitors that have a path to $IP_{V}$ learned from a more preferred neighbor (customers are more preferred than peers, and peers more preferred than providers) than the path to $IP_{H}$ (and vice-versa). Specifically, for each monitor $i\in\mathcal{M}$, calculate the preference of the neighbors for its paths to $IP_{V}$ ($pref\_V_{i}$) and to $IP_{H}$ ($pref\_H_{i}$), and calculate the quantity \begin{equation*}
f_{pref} = \frac{1}{M}\sum_{i\in\mathcal{M}}\mathbb{I}_{pref\_V_{i}>pref\_H_{i}}-\mathbb{I}_{pref\_H_{i}>pref\_V_{i}}
\end{equation*}
where $\mathbb{I}$ the indicator function
\end{enumerate}

\item Use the above quantities as features of a regression model to estimate the hijack impact. Specifically, estimate the hijack impact as
\begin{align*}
\hat{I} &= w_{0} + w_{NIE}\cdot NIE + w_{f}\cdot f
\end{align*}
where $f$ can be $f_{dist}$ or $f_{pref}$, and the weights $w_{0}, w_{NIE}, w_{f}$ are given by Tables~\ref{tab:LRE-parameters-vs-nbMons} and~\ref{tab:LRE-parameters-vs-hijack-types}.
\end{enumerate}
\end{tcolorbox}



\myitem{The biased view of route collectors.} As already discussed, the public monitors are not uniformly deployed in the Internet. This may add bias to the estimations of the NIE in some cases. Consider the following examples:
\footnote{\pavlos{Here we could have a map with the locations of the RIPE and RV route collectors. See
\begin{itemize}
    \item \url{https://www.ripe.net/analyse/internet-measurements/routing-information-service-ris/ris-raw-data}
    \item \url{http://www.routeviews.org/routeviews/index.php/collectors/}
    \item and some code by Petros:
    \item \url{https://github.com/FORTH-ICS-INSPIRE/artemis/blob/master/other/parsers_collectors/parse_collectors.py}
    \item \url{https://github.com/FORTH-ICS-INSPIRE/artemis/blob/master/frontend/webapp/render/static/rrcs_info/collectors_info.json}
\end{itemize}
}}


\textit{Example Scenario 1:} The victim is an AS that is located in a geographical area where many monitors exist, and has short AS-paths (e.g., due to direct peerings) to the the majority of the monitors. These paths are shorter than its average distance among all ASes. At the same time the hijacker AS has longer (than its average) AS-paths to the monitors. In this case, we would expect that the observed impact by the NIE, $\hat{I}_{NIE}$, underestimates the real impact $I$, because the observations $m_{i}$ from the monitors are not representative of the global connectivity of the victim and hijacker.

\textit{Example Scenario 2:} The victim AS happens to be an ISP that is in the customer cone\pavlos{ref} of many monitors. The hijacker's ISP mainly peers with these monitors, and thus its routes are not preferred by them. Then, similarly to the above example, we would expect that $\hat{I}_{NIE}$ underestimates the real impact $I$.

\vkotronis{Need to think also of an overestimation scenario for balance. Maybe simply mention that these cases, when reversed, can lead to respective impact overestimations.}

Generalizing the above examples, the NIE can be biased when the monitors tend to prefer the routes of the victim or the hijacker in a way not representative of the overall behavior of all the other ASes in the Internet. 

\myitem{De-biasing the hijack impact estimation.} The preference of routes from an AS/monitor to another AS is mainly based on inter-AS relationships and path distances in terms of AS hops (see BGP best path selection algorithm~\cite{ciscobestpath}). Note that this information is contained in the AS paths seen by the monitors to the victim and hijacker ASes, and that these AS paths are made available by the feed provided by the RC monitors (i.e., the RIPE RIS and RouteViews public monitoring services with route collectors).

Hence, we suggest that it may be possible to exploit information about AS-relationships and path distances to (i) identify the bias in the hijack estimation and (ii) take them into account to de-bias the estimations of the NIE (i.e., improve its accuracy). To this end, in the following we design a methodology that receives as input information about the AS-relationships of monitors and their distances to the victim and hijacker ASes, and returns an estimation for the hijack impact. 

Specifically, we select to investigate a methodology based on statistical learning models, which learn from the input data (NIE, AS-relationships, path distances) and the hijack impact $I$ in a set of simulated scenarios, and fine-tune a model that predicts the impact based on the input data, i.e., $\hat{I} = f(NIE, AS-relationships, path~distances)$ for a \{V,H\} pair and a set of monitors%
\footnote{An alternative would be to follow a two-stage modeling approach, by first building a model to calculate the bias based on the input data, and then another model that takes as input the calculated bias and provides an impact estimation. While this approach could be amenable to analytical modeling techniques, it could also introduce inaccuracies since it would require modeling, learning, and/or approximations in two stages (instead of one we do now). We defer the investigation of the involved trade-offs and the design of this approach for a future work, and we briefly discuss some possible initial steps towards this direction in Section~\ref{sec:discussion}.}%
.


\subsection{Designing an ML-based Hijack Impact Estimator}

\myitem{Selecting the features.} 
The candidate features for the estimation methodology, need to be quantities that relate to the routing decisions and can be measured or calculated from the available data. Therefore, first, the routing decisions of an AS mainly depend on the local routing polices (e.g., preference of neighboring ASes) and path lengths. Second, the available information that is related to the routing decisions is (i) the \textit{sequence of AS-links} in the AS-paths and (ii) the \textit{length of the AS-paths} observed and provided by the monitors, as well as (iii) the \textit{AS-relationships} (as they are inferred in the CAIDA AS-relationship dataset~\cite{AS-relationships-dataset, AS-relationships-IMC-2013}) of the ASes involved in the seen AS-links, which can be used to approximately capture the --typically not known/disclosed-- AS routing policies/preferences. \vkotronis{The 3rd point might need to be put at a higher place, it takes precedence in the route selection process, correct? Or rephrase the as-link selection as the first point.}

In this context, to compile the needed data, we collect for each monitor its best paths to: (a) a prefix $IP_{V}$ announced by the victim AS, (b) a prefix $IP_{H}$ announced by the hijacker AS, and (c) the hijacked prefix $IP_{*}$ (which is announced by both ASes). For all these collected paths, we calculate the following quantities: (i) the path length, (ii) the AS-relationship between the monitor and the next AS in the path, (iii) the type, direction and sequence of AS-relationships in the entire path. Also, from the path to the hijacked prefix, we find (iv) whether the monitor is infected. 

From these quantities, we build a number of features to be fed in the predictive models for the hijack impact: 
\begin{itemize}[leftmargin=*]
\item average path lengths to victim/hijacker
\item number of monitors with shorter paths to victim/hijacker
\item number of monitors with a path to victim/hijacker through a customer/peer/provider neighbor
%\item number of monitors with a path to victim through a neighbor with lower/equal/higher preference than the neighbor in the path to the hijacker
\item number of monitors for which the \textit{entire path} to victim is less/ equally/more preferable than the path to the hijacker  (as calculated using the AS-relationships in the entire path and the catchment inference methodology of~\cite{sermpezis2019pomacs})
\item number of infected monitors (i.e., NIE)
\end{itemize}
as well as \textit{combinations of all the above features / sets of monitors}; e.g., number of infected monitors with equal preference neighbors to victim/hijacker and shorter path to victim.


We simulate hijack scenarios with different \{V,H\} pairs, and for each scenario we calculate the above features and the total hijack impact that is used for training and testing the models. We test a number of machine-learning regression models (see below for details), which receive as input (all or a subset of) the above features and fit their hyper-parameters using the training samples for the total hijack impact. 

When using all the features, we achieve the best accuracy. However, we found that the contribution of several features is negligible, either as individual features and/or when used in combination with other features. Removing gradually the unimportant features and merging features, we resulted in a small set of features, with which the predictive models achieve practically the same accuracy as in the best case (using all features)\footnote{We omit the details of the feature elimination process due to space limitation, and because its steps do not add significant value to the main findings of the paper.}. Specifically, we identified two subsets of features that achieve the best accuracy:
\begin{itemize}[leftmargin=*]
\item \textbf{\textit{Feature set 1: NIE, $\mathbf{f_{dist}}$}}
\begin{itemize}
    \item fraction of infected monitors, i.e., the NIE, $\frac{1}{M}\sum_{i\in\mathcal{M}}m_{i}$
    \item fraction of monitors with \textit{shorter} paths to the \textit{victim}
    \item fraction of monitors with \textit{shorter} paths to the \textit{hijacker}
\end{itemize}
We merge the latter two quantities in a single feature\footnote{The rationale behind this choice is that we observed in several ML-models that the coefficients of these two features, $\frac{1}{M}\sum_{i\in\mathcal{M}}\mathbb{I}_{dist\_V_{i}<dist\_H_{i}}$ and $\frac{1}{M}\sum_{i\in\mathcal{M}}\mathbb{I}_{dist\_H_{i}<dist\_V_{i}}$, were approximately opposite numbers \vkotronis{what do you mean with ``opposite'' numbers?}, thus meaning that their difference can be used as a single feature (which we verified also with accuracy tests).}:
\begin{equation*}
\textstyle{f_{dist} = \frac{1}{M}\sum_{i\in\mathcal{M}}\mathbb{I}_{dist\_V_{i}<dist\_H_{i}}-\mathbb{I}_{dist\_H_{i}<dist\_V_{i}}}
\end{equation*}
where $\mathbb{I}_{x}=1$ if $x$ is true and $\mathbb{I}_{x}=0$ otherwise.

\item \textbf{\textit{Feature set 2: NIE, $\mathbf{f_{pref}}$}}
\begin{itemize}
    \item fraction of infected monitors, i.e., the NIE, $\frac{1}{M}\sum_{i\in\mathcal{M}}m_{i}$
    \item fraction of monitors with higher \textit{preference} to the neighbor in the path to the \textit{victim} (than the neighbor to the hijacker path)
    \item fraction of monitors with higher \textit{preference} to the neighbor in the path to the \textit{hijacker} (than the neighbor to the victim path)
\end{itemize}
We merge the latter two quantities in a single feature:
\begin{equation*}
\textstyle{f_{dist} = \frac{1}{M}\sum_{i\in\mathcal{M}}\mathbb{I}_{pref\_V_{i}>pref\_H_{i}}-\mathbb{I}_{pref\_H_{i}>pref\_V_{i}}}
\end{equation*}
\end{itemize}


For instance, let us denote with $i$, $V$, and $H$ the ASNs of the monitor $i$, the victim $V$, and the hijacker $H$, respectively, and assume that the best paths of the monitor $i$ to a prefix $IP_{V}$ announced by the AS $V$, and to a prefix $IP_{H}$ announced by the AS $H$ (this is not the hijacked prefix, but a prefix owned and legitimately announced the AS $H$), are
\begin{align*}
 path(IP_{V}) &= [i, AS1, AS2, V]   \\
 path(IP_{H}) &= [i, AS3, AS4, AS5, H]
\end{align*}
and that \textit{AS1 is a provider of $i$} and \textit{AS3 a peer of $i$}. Then, the path lengths of the monitor to the victim and hijacker are $dist\_V_{i} = 3$ and $dist\_H_{i} = 4$, respectively, and for the preference of the neighbors for these paths it holds $pref\_V_{i} > pref\_H_{i}$.

\myitem{Selecting the model.} Having selected the feature sets, we proceed to the selection of the predictive model\footnote{In practice the feature and model selection processes took place simultaneously, through continuous feedback and optimization cycles; here, we discuss them separately only for the sake of presentation.}. We tested a number of regression models, whose output can be a continuous value in [0,1] (i.e., as the hijack impact is). Table~\ref{tab:rmse-ml-models} presents the RMSE for the best performing models among those we tested. 


\begin{table}[h]
\centering
\caption{RMSE of different regression models for the two selected feature sets.}
% \caption{RMSE of different regression models (rows), using different AS-path properties (columns) and the NIE as features.}
\label{tab:rmse-ml-models}
\begin{tabular}{l|ccc}
{}       & \multicolumn{2}{c}{Feature sets}\\
Regression Models       & \{NIE, $f_{dist}$\} & \{NIE, $f_{pref}$\}\\
\hline
Linear                  & \textbf{7.4\%}     & 7.9\%\\
Support Vector          & 7.7\%     & 7.9\%\\
k Nearest Neighbors (k=10)       & 8.1\%        & 7.9\%\\
Decision Tree (max depth=5)           & 8.0\%   & 8.1\%\\
MLP (NN=(64,64), ReLU) & \textbf{7.4\%}   &\textbf{7.4\%}
\end{tabular}
% \begin{tabular}{l|ccc}
% {}       & \multicolumn{3}{c}{Features}\\
% Regression Models       & distances & AS-rel. & dist. \& AS-rel.\\
% \hline
% Linear                  & \textbf{7.4\%}     & 7.9\%    & 8.3\%\\
% Support Vector          & 7.7\%     & 7.9\%    & 8.3\%\\
% k Nearest Neighbors (k=10)       & 8.1\%        & 7.9\%     & 8.3\%\\
% Decision Tree (depth=5)           & 8.0\%   & 8.1\%    & 8.6\%\\
% MLP (NN=(64,64), ReLu) & \textbf{7.4\%}   &\textbf{7.4\%}    & 8.2\%\\
% \end{tabular}
\end{table}


For both feature sets, the Multi-layer perceptron (MLP) regressor, using a neural networks with two layers of 64 nodes each and ReLU activation functions, achieves the lowest RMSE (0.074 or 7.4\%). We can also see that the linear regression model with the feature set \{NIE, $f_{dist}$\} is equally accurate. This is an important finding, since it shows that the best accuracy can be achieved even by using a simple and interpretable model%
\footnote{It also indicates that the features \textit{NIE} and $f_{dist}$ (and similarly for the $f_{pref}$) affect in a linear way the predictions. This can be clearly seen in Fig.~\ref{fig:ML-2D-visualization-Impact-closeness} in Appendix~\ref{appendix:visualization-ML-boundaries} \pavlos{plot the same plot for the correct features and model} where we present the predictions of the MLP model, $\hat{I}=g(NIE,f_{dist})$, which show that the function $g$ can be approximated with a linear function (i.e., as in the case of the linear regression model).}%
. Interpretable models come with a number of advantages, which make them preferable (e.g., compared to deep learning techniques that typically are considered as black-boxes \vkotronis{very nice argument!!!}) and is in line with the recent efforts for explainable ML models and AI algorithms~\cite{weld2019challenge}. 

Specifically, using a linear regression model (i) can help towards understanding of the bias introduced by the deployment of the RC monitors and how it can be mitigated, and thus (ii) it can provide insights for future (analytic) modeling efforts; moreover, (iii) it is simple to implement and adapt, for example, to fine-tune the model using data from real hijacking events whose impact is measured (e.g., from ongoing activities to create a database about hijacking events\pavlos{cite observatory}) or to adapt the model for different hijack settings (e.g., adapting it per AS / potential victim, or focusing on the case of ASes known as serial hijackers~\cite{testart2019profiling}\footnote{In the former example one can simulate hijacks towards the given AS by considering different ASes, and in the latter example, simulate hijacks from one of the serial hijackers and randomly selecting victim.}).


To this end, we select to use the linear regression models as estimators for the hijack impact; in the remainder we refer to these models as the Linear Regression Estimators (LRE). Note that we select to use the LRE also in the case of the second feature set \{NIE, $f_{pref}$\}, where its accuracy is lower but comparable to the corresponding MLP model (RMSE 7.9\% vs. 7.4\% - see Table~\ref{tab:rmse-ml-models}). The LRE model estimates the hijack impact as follows
\begin{equation}
\hat{I}_{LRE} = w_{0} + w_{NIE}\cdot NIE + w_{f}\cdot f 
\end{equation}
where $f$ is either $f_{dist}$ or $f_{pref}$, depending on the selected feature set. Table~\ref{tab:LRE-parameters-vs-nbMons-vs-hijackTypes} gives the values for the weights / model parameters $w_{0}$, $w_{NIE}$, and $w_{f}$, fitted on simulation results over 1000 randomly selected \{V,H\} pairs.


%%%%%%%%%%%%%%%%% ONE TABLE - SMALL VERSION %%%%%%%%%%%%%%%%%%%%%
\begin{table}[h]
%\centering
\caption{Model parameters of LRE vs. number of monitors (for hijack Type-0) and vs. hijack types (for all RC monitors).}
\label{tab:LRE-parameters-vs-nbMons-vs-hijackTypes}
\begin{tabular}{cl|cccc||cc}
{}&{}          & \multicolumn{4}{c}{\#monitors M}& \multicolumn{2}{c}{Hijack Type}\\
\multicolumn{2}{c|}{Parameters}    &{10}& {50}& {100}& {229}&{1}& {2}\\
\hline
\multirow{3}{*}{\shortstack{LRE\\($f_{pref}$)}}
&$w_{0}$   &{0.14}& {0.06}& {0.04}& {0.04}
    & {0.02}& {0.01}\\
&$w_{NIE}$ &{0.73}& {0.88}& {0.91}& {0.92}
    & {0.84}& {0.81}\\
&$w_{f}$   &{0.03}& {0.10}& {0.11}& {0.11}
    & {0.05}& {0.01}\\
\hline
\multirow{3}{*}{\shortstack{LRE\\($f_{dist}$)}}
&$w_{0}$  &{0.17}& { 0.13}& { 0.12}& { 0.12}
    & { 0.04}& { 0.02}\\
&$w_{NIE}$&{0.67}& { 0.74}& { 0.76}& { 0.77}
    & { 0.80}& { 0.80}\\
&$w_{f}$  &{0.05}& {0.08}& {0.08}& {0.08}
    & {0.04}& { 0.00}\\
\end{tabular}
\end{table}
%%%%%%%%%%%%%%%%% [END] ONE TABLE - SMALL VERSION %%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%% ONE TABLE - FULL VERSION %%%%%%%%%%%%%%%%%%%%%
% \begin{table*}[h]
% %\centering
% \caption{Model parameters of LRE vs. number of monitors (for hijack Type-0) and vs. hijack types (for all RC monitors).}
% \label{tab:LRE-parameters-vs-nbMons}
% \begin{tabular}{cl|cccccc||ccc}
% {}&{}          & \multicolumn{6}{c}{\#monitors (M)}& \multicolumn{3}{c}{Hijack Type}\\
% \multicolumn{2}{c|}{Parameters}    & {229}& {100}& {50}& {20}& {10}& {5} 
%     & {0}& {1}& {2}\\
% \hline
% \multirow{3}{*}{\shortstack{LRE\\($f_{pref}$)}}
% &$w_{0}$   & {0.04}& {0.04}& {0.06}& {0.09}& {0.14}& { 0.19}
%     & {0.04}& {0.02}& {0.01}\\
% &$w_{NIE}$ & {0.92}& {0.91}& {0.88}& {0.81}& {0.73}& { 0.63} 
%     & {0.92}& {0.84}& {0.81}\\
% &$w_{f}$   & {0.11}& {0.11}& {0.10}& {0.06}& {0.03}& { 0.04}
%     & {0.11}& {0.05}& {0.01}\\
% \hline
% \multirow{3}{*}{\shortstack{LRE\\($f_{dist}$)}}
% &$w_{0}$  & { 0.12}& { 0.12}& { 0.13}& { 0.14}& { 0.17}& { 0.22}
%     & { 0.12}& { 0.04}& { 0.02}\\
% &$w_{NIE}$& { 0.77}& { 0.76}& { 0.74}& { 0.72}& { 0.67}& { 0.58} 
%     & { 0.77}& { 0.80}& { 0.80}\\
% &$w_{f}$  & {-0.08}& {-0.08}& {-0.08}& {-0.07}& {-0.05}& {-0.05} 
%     & {-0.08}& {-0.04}& { 0.00}\\
% \end{tabular}
% \end{table*}
%%%%%%%%%%%%%%%%% [END] ONE TABLE - FULL VERSION %%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%% TWO TABLES - FULL VERSION %%%%%%%%%%%%%%%%%%%%%
% \begin{table}[h]
% \centering
% \caption{Model parameters of LRE vs. number of monitors.}
% \label{tab:LRE-parameters-vs-nbMons}
% \begin{tabular}{cl|cccccc}
% {}&{}          & \multicolumn{6}{c}{\#monitors (M)}\\
% \multicolumn{2}{c|}{Parameters}    & {229}& {100}& {50}& {20}& {10}& {5} \\
% \hline
% \multirow{3}{*}{\shortstack{LRE\\(AS-rel)}}
% &$w_{0}$   & {0.04}& {0.04}& {0.06}& {0.09}& {0.14}& { 0.19}\\
% &$w_{NIE}$ & {0.92}& {0.91}& {0.88}& {0.81}& {0.73}& { 0.63} \\
% &$w_{f}$   & {0.11}& {0.11}& {0.10}& {0.06}& {0.03}& { 0.04} \\
% \hline
% \multirow{3}{*}{\shortstack{LRE\\(dist)}}
% &$w_{0}$  & { 0.12}& { 0.12}& { 0.13}& { 0.14}& { 0.17}& { 0.22}\\
% &$w_{NIE}$& { 0.77}& { 0.76}& { 0.74}& { 0.72}& { 0.67}& { 0.58} \\
% &$w_{f}$  & {-0.08}& {-0.08}& {-0.08}& {-0.07}& {-0.05}& {-0.05} \\
% \end{tabular}
% \end{table}

% \begin{table}[h]
% \centering
% \caption{Model parameters of LRE vs. hijack types.}
% \label{tab:LRE-parameters-vs-hijack-types}
% \begin{tabular}{cl|cccccc}
% {}&{}          & \multicolumn{3}{c}{Hijack Type}\\
% \multicolumn{2}{c|}{Parameters}    & {0}& {1}& {2}\\
% \hline
% \multirow{3}{*}{\shortstack{LRE\\(AS-rel)}}
% &$w_{0}$   & {0.04}& {0.02}& {0.01}\\
% &$w_{NIE}$ & {0.92}& {0.84}& {0.81}\\
% &$w_{f}$   & {0.11}& {0.05}& {0.01}\\
% \hline
% \multirow{3}{*}{\shortstack{LRE\\(dist)}}
% &$w_{0}$  & { 0.12}& { 0.04}& { 0.02}\\
% &$w_{NIE}$& { 0.77}& { 0.80}& { 0.80}\\
% &$w_{f}$  & {-0.08}& {-0.04}& { 0.00}\\
% \end{tabular}
% \end{table}
%%%%%%%%%%%%%%%%% [END] TWO TABLES - FULL VERSION %%%%%%%%%%%%%%%%%%





The accuracy of the LRE models is compared with the NIE in Tables~\ref{tab:rsme-nie-lre-vs-nbMons}\pavlos{maybe plot this in a figure} (vs. the number of monitors $M$) and~\ref{tab:rmse-vs-hijack-NIE-ML} (vs. the hijack type). When considering all RC monitors, the RMSE of NIE is reduced from $10\%$ to $7.4\%$ $7.9\%$ with LRE($f_{dist}$) and LRE($f_{pref}$), which is a relative improvement of 20\%-25\%. A similar relative improvement can be observed for all values of $M$ and all hijack types, indicating that the LRE can consistently improve the estimation accuracy.


\begin{table}[h]
\centering
\caption{RMSE of NIE and the Linear Regression estimator (LRE) vs. number of monitors.}
\label{tab:rsme-nie-lre-vs-nbMons}
\begin{tabular}{l|rrrrrr}
{}          & \multicolumn{6}{c}{\#monitors (M)}\\
Estimator   & {5}& {10}& {20}& {50} & {100}& {229}\\
\hline
NIE         & {19.4\%} & {16.0\%}& {13.1\%}& {11.6\%}& {10.5\%}& {10.0\%}\\
LRE(AS-rel) & {15.0\%}& {12.7\%}& {10.7\%}& { 9.2\%}& { 8.4\%}& { 7.9\%}\\
LRE(dist)   & {14.7\%}& {12.4\%}& {10.4\%}& { 8.8\%}& { 8.0\%}& { 7.4\%}
\end{tabular}
\end{table}




\begin{table}[h]
\centering
\caption{RMSE vs. hijack Type}
\label{tab:rmse-vs-hijack-NIE-ML}
\begin{tabular}{l|rrr}
Model       & Type-0    & Type-1 & Type-2\\
\hline
NIE         &{10.0\%} &{9.6\%} &{8.9\%}\\
LRE (AS-rel)&{ 7.9\%} &{6.7\%} &{5.5\%}\\
LRE (dist)  &{ 7.4\%} &{6.6\%} &{5.5\%}
\end{tabular}
\end{table}




\myitem{Interpreting the model.} The linear combination of the features in LRE, enables us to understand the role of each feature from the value of the weights in Table~\ref{tab:LRE-parameters-vs-nbMons-vs-hijackTypes}. In both LRE models, we can see that: (i) NIE plays the major role, by contributing around 70\%-90\% in the prediction. This was expected qualitatively (the values of $w_{NIE}$ quantify its role), since the NIE already can estimate the impact to a certain accuracy, and our goal is just to ``correct'' it and improve its estimations. The role of NIE increases with $M$, where the estimation becomes more robust (see Fig.~\ref{fig:RMSE-NIE-random-RC-RA-vs-nb-monitors-Type0}), while for small $M$ the ``corrections'' in the NIE are larger. (ii) There is a constant factor that contributes around 10\%, i.e., even if none of the measured monitors was infected, the LRE would predict an impact of $w_{0}$. While this term is seemingly counter-intuitive, it corresponds to the (average) value of the impact not seen by any RC monitors; in fact, we tested linear regression models where we forced $w_{0}=0$, and we observed higher RMSE values, thus verifying the role of this constant implicit impact. Moreover, the less the monitors, the higher the probability that none of the $M$ monitors is infected, which explains that $w_{0}$ increases for lower values of $M$. (iii) Both the features $f_{dist}$ and $f_{pref}$, indicate how ``preferrable'' by the RC monitors is the route to the victim compared to the hijacker's route: the higher the value of the feature, the more ``preferred'' is the victim route by the monitors, and thus the more probable is that the impact is underestimated. Hence, the weights $w_{f}$ are positive, to ``correct'' this underestimation. The contribution of $f_{dist}$ and $f_{pref}$ is around 8\% and 10\%, respectively.

\vkotronis{Regarding $f_{pref}$, is it simply a convention that we explain it from the victim's perspective, or sth else? For example, couldn't we interpret this from the hijacker's perspective too? Also, why don't we use both $f_{dist}$ and $f_{pref}$ within the regressor's formula?}


\myitem{Practical Implementation.}
The LRE requires as input information (i) the NIE and (ii) the quantity $f_{dist}$ or $f_{pref}$. 

The NIE is the number \vkotronis{isn't ``fraction'' the correct term here?} of RC monitors that have selected a path to the hijacker for the hijacked prefix $IP_{*}$. The paths of the RC monitors to $IP_{*}$ can be retrieved in real-time from the RIPE RIS service~\cite{ripe-ris-real-time}\pavlos{update reference}, which provides a live feed of the BGP updates received by the RIS route collectors, while some route collectors of RouteViews already provide live BGP feeds as well \vkotronis{hmmm I do not know about this, did Alistair or Alberto inform you?}. There are open-source tools that automate and facilitate the process of continuously monitoring paths to a prefix: CAIDA's BGPStream~\cite{bgpstream-website, bgpstream-paper}, ARTEMIS~\cite{artemis-website, sermpezis2018artemis}, \pavlos{the tool by Job Sneider?~\cite{}} \vkotronis{yes this is the BGPalerter, I will add a ref later; however, it is essentially a RIS live feed}.

To calculate the quantities $f_{dist}$ and $f_{pref}$, we need to know the paths selected by monitors to a prefix announced only by the victim AS ($IP_{V}$) and a prefix announced only by the hijacker AS ($IP_{V}$)\footnote{We remind here that these quantities cannot be calculated from the paths to $IP_{*}$, because each monitor has only one path to $IP_{*}$ (either to the victim or hijacker AS), and thus we cannot know, e.g., to which of the two ASes it is closer (i.e. we would know only $dist\_V{i}$ or $dist\_V{i}$ \vkotronis{sth is wrong here, you mean the hijacker?}, but not both).}. \vkotronis{Do you need $IP_{*}$ (by victim or hijacker) being actually announced by them, or would it also suffice to see them in paths also to other prefixes (e.g, on-path as transits)? These paths would be much more frequent, especially for actual transit victims.} In practice, this can be implemented by building and maintaining for each monitor $i$ a dictionary with the distances $dist\_X_{i}$ and $pref\_X_{i}$, for every AS $X$ \vkotronis{that they observe in the received BGP advertisement \texttt{AS-PATH}s}. The quantities $dist\_X_{i}$ and $pref\_X_{i}$ can be calculated from the paths in the RIB of the monitor $i$, which can be retrieved from CAIDA's BGPStream~\cite{bgpstream-website, bgpstream-paper} or from the MRT files provided by the RIPE RIS and RouteViews projects.

\vkotronis{Don't you need more info sources too like CAIDA's AS-rel, etc.?}

\pavlos{It would be great, if we could implement this in a script (e.g., which could be used later in Artemis). @Vasilis: what is the estimated effort for this? who could implement this? Do you think it would be possible to have it by the camera ready (early May)?}

\vkotronis{This seems quite easy; just instruct BGPStream to query the RIBs and retrieve these quantities using additional sources like AS-rel if required. Implementing this as a continuous monitoring mechanism would require a bit more effort (and connection with newer AS-rel snapshots from CAIDA), but it can be a new microservice to be integrated later in ARTEMIS. I would implement this as a container that does a very specific job. The effort would be 3-4 days, but we need to discuss the design requirements carefully, Regarding who: on my side, it depends on my availability since I will be at the army starting on Jan the 10th. If time permits, I can try making a pass till Christmas, but cannot guarantee availability. Kostas or George Epta could also take a look at this, if they have time, it is not sth extremely challenging if they have 4 days to work on it (1 design, 1 impl, 1 testing, 1 re-impl and re-testing).}.





==> ML_estimator_preliminaries_discussion.tex <==

However, the ping campaign methodology is still not applicable in the case of MitM attacks; also, it requires active measurements which add a small extra overhead (e.g., deployment of a system to trigger and monitor the pings). Hence, as an alternative (and/or for completeness), we design a methodology based on control-plane \vkotronis{why not also data-plabe (RA)?} information from monitors of the public services. The public services methodology needs to overcome some challenges and limitations that have been indicated by our analysis (e.g., lower accuracy - Fig.~\ref{fig:RMSE-NIE-rnd-RC-RA-vs-nb-monitors}) and are discussed in more detail below.

\myitem{Public services: challenges and limitations.} There are two types of monitors that can be considered in this approach: RC and RA. As is shown in Fig.~\ref{fig:RMSE-NIE-rnd-RC-RA-vs-nb-monitors}, both sets of monitors achieve similar accuracy, with RA achieving at most only 0.01 lower RMSE than RC (despite the fact that there exist one order of magnitude more RA monitors than RC monitors). However, conducting measurements with RC has a number of advantages (low overhead, real-timeness) compared to RA measurements: RC monitors continuously provide a \textit{real-time} feed of control-plane data (passive measurement) through existing tools and interfaces (such as, RIPE RIS~\cite{add-citation}, BGPStream~\cite{bgpstream-website}, ARTEMIS~\cite{artemis-website,sermpezis2018artemis}), and --in contrast to RA-- do not require to conduct active measurements (traceroutes) upon the detection of a hijack. Adding to this, a limitation of the RA measurements is that depending on the type of the hijack (e.g., in MitM), traceroute measurements may require to map the data plane information to AS-level information. i.e., map IP addresses in the traceroute path to ASNs. However, this mapping is not always possible (e.g., IP interfaces not replying, resulting in incomplete paths with stars ``*'') and/or is known to be often inaccurate\pavlos{[REFs]}, which can ultimately lead to wrong measurements and thus increase of the estimation error. For these reasons, we choose to design a methodology based on control-plane measurements using the RC monitors (nevertheless, our methodology can still be applied with the RA monitors).

\vkotronis{We can also mention that traceroutes give as end-to-end path information, when the path is complete and the mapping accurate, but this accuracy and completeness are very hard to attain. Also we may need to hint at possible inconsistencies between the control and data plane, which is very common in practice (ref needed, you can also ping Lefteris on this).}

The aim of our methodology is to improve the accuracy of the NIE with RC. To this end, we build on the fact that \textit{RC measurements provide richer information than simply measuring whether the monitor is infected}. Specifically, RC monitors provide BGP updates, including the entire AS-path, which contains richer information relating to Internet routes, such as AS-links and path lengths. In other words, RC provide implicit information about why the monitors selected a route to the victim or hijacker AS. As shown, when knowing the routing policies and topology (R-graph) we can achieve very high accuracy. Hence, our methodology is based on the idea that we can exploit the information about routing policies and topology contained in RC measurements (AS-links and path lengths), to achieve higher accuracy. We design our methodology in Section~\ref{sec:ml-estimator} where we study different approaches and statistical models to estimate the hijack impact.




==> NIE_with_RGraph.tex <==

The methodology we propose uses information (i) provided by RC monitors about the AS-paths to the victim and hijacker ASes, and (ii) about AS routing policies, to adapt the estimations of NIE-RC towards more accurate estimations \vkotronis{The latter needs some rephrasing I think}. It is summarized as follows:

\begin{tcolorbox}
\textbf{LRE-RC: Hijack impact estimation from route collectors measurements.}

\pavlos{TODO}
\end{tcolorbox}



\myitem{The biased view of route collectors.} As already discussed, the public monitors are not uniformly deployed in the Internet. This may add bias to the estimations of the NIE in some cases. Consider the following examples:
\footnote{\pavlos{Here we could have a map with the locations of the RIPE and RV route collectors. See
\begin{itemize}
    \item \url{https://www.ripe.net/analyse/internet-measurements/routing-information-service-ris/ris-raw-data}
    \item \url{http://www.routeviews.org/routeviews/index.php/collectors/}
    \item and some code by Petros:
    \item \url{https://github.com/FORTH-ICS-INSPIRE/artemis/blob/master/other/parsers_collectors/parse_collectors.py}
    \item \url{https://github.com/FORTH-ICS-INSPIRE/artemis/blob/master/frontend/webapp/render/static/rrcs_info/collectors_info.json}
\end{itemize}
}}


\textit{Example Scenario 1:} The victim is an AS that is located in a geographical area where many monitors exist, and has short AS-paths (e.g., due to direct peerings) to the the majority of the monitors. These paths are shorter than its average distance among all ASes. At the same time the hijacker AS has longer (than its average) AS-paths to the monitors. In this case, we would expect that the observed impact by the NIE, $\hat{I}_{NIE}$, underestimates the real impact $I$, because the observations $m_{i}$ from the monitors are not representative of the global connectivity of the victim and hijacker.

\textit{Example Scenario 2:} The victim AS happens to be an ISP that is in the customer cone\pavlos{ref} of many monitors. The hijacker's ISP mainly peers with these monitors, and thus its routes are not preferred by them. Then, similarly to the above example, we would expect that $\hat{I}_{NIE}$ underestimates the real impact $I$.

\vkotronis{Need to think also of an overestimation scenario for balance. Maybe simply mention that these cases, when reversed, can lead to respective impact overestimations.}

Generalizing the above examples, the NIE can be biased when the monitors tend to prefer the routes of the victim or the hijacker in a way not representative of the overall behavior of all the other ASes in the Internet. 

\myitem{De-biasing the hijack impact estimation.} The preference of routes from an AS/monitor to another AS is mainly based on inter-AS relationships and path distances in terms of AS hops (see BGP best path selection algorithm~\cite{ciscobestpath}). Note that this information is contained in the AS paths seen by the monitors to the victim and hijacker ASes, and that these AS paths are made available by the feed provided by the RC monitors (i.e., the RIPE RIS and RouteViews public monitoring services with route collectors).

Hence, we suggest that it may be possible to exploit information about AS-relationships and path distances to (i) identify the bias in the hijack estimation and (ii) take them into account to de-bias the estimations of the NIE (i.e., improve its accuracy). To this end, in the following we design a methodology that receives as input information about the AS-relationships of monitors and their distances to the victim and hijacker ASes, and returns an estimation for the hijack impact. 

Specifically, we select to investigate a methodology based on \pavlos{... TODO ...} 






==> discussion.tex <==
\begin{itemize}
\item Based on the analytic results of Section~\ref{sec:ping-estimator}, we can transform the NIE-ping to an unbiased estimator: the new unbiased estimator will be $\hat{I} = \frac{NIE-p}{1-p}$ and its expected value is $E[\hat{I}]=I$; see proof of Theorem~\ref{}. However, a technical challenge is that this requires to (continuously) know the failure probability $p$; this could be done with keeping track of the reponse probabilities of IP addresses \pavlos{is this in the ANT dataset?}. In principle this will reduce bias and RMSE, however, the effect of inaccurate estimation of $p$ needs to be taken into account (e.g., take care of the case that an inaccurate estimation of $p$ leads to a worse RMSE of NIE-ping).

\item Quantify impact estimation accuracy per regions. E.g., what is the accuracy for hijacks from region A (to victims in region B)? Are there significant differences among regions? In particular for the RC case, where it is known that RCs are not uniformly deployed all over the world. Could/should we modify the methods and create per-region methods?

\item Some ASes may route to different origins from different ingress points. \pavlos{quantify this from 2006 paper (see sigmetrics paper) and Verfploeter}. How to take this into account. (small impact difference?)

\item \pavlos{TODO: discuss about system aspects of pinging system}

\vkotronis{Experiment support for TCP probes on well-known ports}

\vkotronis{Experiment with given population of ASes to derive pingability}

\vkotronis{Btw we can do similar campaigns with DP probes on e.g., TCP or UDP ports; maybe we do not have to constrain our approach to pings (or we can mention this in the discussion section). We do not have to actually do them, but we can claim that we can do them; the code supports them and the end result format is exactly the same.}


\item \pavlos{Accuracy of impact estimation over time. Maybe cite ARTEMIS results (Fig 7b) about nb of monitors seen the hijack over time. It seems that almost all monitors see the event within a minute. We can check this with our data as well.}
\end{itemize}


\pavlos{Maybe add simple rule that: (i) if we know the ping failure probability of the IP addresses $p_{IP}$, and (ii) conduct $N_{IP}$ measurements per AS, then to achieve a certain probability of at least one failure, i.e., the probability $p$, we need to do $N_{IP}\geq \frac{\log{p}}{\log{p_{IP}}}$ pings per AS.}

==> experiments_backup_26Jan2020.tex <==
We conduct controlled hijacking experiments in the real Internet using the PEERING testbed~\cite{schlinker2014peering,peering}.
The PEERING testbed owns ASNs and IP prefixes and has BGP connections with operational networks in several locations (\emph{sites}) around the world. 

The hijacking experiments\footnote{Our experiments took place within Nov.-Dec. 2019.} consist of the following steps.

\myitem{Selection of \{V,H\} pair.} We create two virtual ASes, assign to them the ASNs $61574$ and $61575$, and connect them to two distinct sites of the PEERING testbed. We select one of them to be the victim AS (V) and the other the hijacker AS (H).

%\item \textbf{Beacon BGP announcements:} We announce through BGP a prefix from V, wait 30min for the announcement to propagate to the entire Internet, and then withdraw the prefix. We do the same for H as well. This step is needed to obtain information about the best paths of the monitors (RC) towards V and H.

\myitem{BGP announcements and Hijacking.} We announce the prefix $184.164.243.0/24$ from V, and wait 30min for the convergence of the BGP announcement. Then, we hijack the prefix (i.e., announce the same prefix) from H.

\myitem{Impact measurement.} To measure the impact of the hijack, we perform a ping campaign (see details in Section~\ref{sec:ping-campaign}): We select 46k ASes and ping an IP address in each of them. We monitor through which PEERING site the ping reply returns: if it returns through the H (or, V) site, we consider the corresponding AS as infected (or, not infected). We use this information as the ground truth for the hijack impact of each experiment.
%
Moreover, to apply our impact estimation methodologies, we conduct data-plane (traceroutes) and control-plane (BGP updates) measurements after the hijacking announcement (Section~\ref{sec:public-measurements}), from which we infer whether the monitors (RIPE Atlas probes or peers of the route collectors) route their traffic to the H or the V site.

%\textit{Remark:} The extensive ping campaign provides detailed information, which we use as ground truth for the impact; however, it is a heavyweight process (wrt. to time needed and number of measurements) and cannot be used for a timely impact estimation in practice. 


\subsection{Ping Campaign}\label{sec:ping-campaign}
We issue ICMP pings from a client (i.e., a local machine) within the PEERING testbed towards reachable IP addresses in $46k$ ASes in the Internet, and monitor whether the ping replies return through the victim or the hijacker PEERING sites. 

Specifically, we first compile a list of pingable IP addresses per ASN, by combining the following two datasets.
\begin{itemize}[leftmargin=*]
\item \textbf{Prefix-to-AS mapping:} We consider information from the RIPE RIS~\cite{riperis} (via the RIPEstat API~\cite{ripestat}) and RouteViews~\cite{routeviews} (via CAIDA's \texttt{pfx2as}~\cite{caidapfx2as}) projects. These datasets map IP prefixes announced in BGP to the ASN that originates them. We filter out mappings that appear to be inconsistent within a period of a month (e.g., due to transient incidents), and merge the two datasets.

\item \textbf{IP hitlists from ANT Lab}~\cite{antlabhitlists}: These are lists of IP addresses that are found to be reachable via \texttt{ping} with high probability, based on past measurements. We select only the IP addresses with more than 90\% confidence score. 
\end{itemize}

Then, we send an ICMP echo request packet out of our PEERING client to each IP address in our dataset, and monitor the replies. In case an ICMP echo reply packet comes back by re-entering PEERING and reaching our client, we monitor out of which ingress PEERING-facing tunnel interface the client received it. Resolving this interface to the corresponding PEERING site, we can determine which site (i.e., the victim or the hijacker) attracted the traffic from the pinged AS. 
%This methodology is similar to Verfploeter~\cite{de2017broad}, which focuses though on catchment measurement of a large CDN.




\subsection{Measurements from Public Services}\label{sec:public-measurements}

We conduct control and data plane measurements from the public services to collect the information needed by our impact estimation methodologies.

\myitem{Data-plane measurements.} We employ traceroutes from RIPE Atlas probes towards the announced prefix. To identify to which site (victim or hijacker) the traceroute enters the PEERING testbed, we check in the traceroute the last IP address before it enters PEERING. We map this IP address to an AS (using the above prefix-to-AS dataset), and if the ASN belongs to an upstream provider of the hijacker (victim) site, then we infer that the AS of the RIPE Atlas probe is infected (not infected)\footnote{In case the victim and hijacker sites share an upstream, and the last traceroute hop is mapped to this upstream, then we do not proceed to an inference.}.



\myitem{Control-plane measurements.} We employ CAIDA's BGPStream tool~\cite{caidabgpstream} to collect BGP updates received by RouteViews and RIPE RIS monitors. For each monitor we store the BGP RIBs, and update them (after the hijacking announcement) using the observed BGP updates. From the AS paths in the RIBs, we extract the origin ASNs and use them to infer to which site the monitor AS routes its traffic. For example, from the AS path $[ASX, ASY, \dots, Hijacker\_ASN]$, we infer that the monitor $ASX$ is infected.

\subsection{Results}

We considered a set of 6 PEERING sites that were responsive at the time of our experiments, their BGP announcements propagated to the entire Internet (i.e., were visible by the route collectors), and they were reachable through data-plane measurements (pings, traceroutes) from the majority of ASes in the Internet. 

\pavlos{If we have space we can add a table with the details of the PEERING muxes, e.g., IXP/ISP, \# transits/peers, country, etc. (the list is: amsterdam01, %phoenix01, 
ufmg01, uw01, grnet01, seattle01, clemson01)} 



We considered all possible combinations of pairs \{V,H\} for these sites, and conducted Type-0 hijacking experiments. We omit the experiments in which the hijack impact was trivial ($100\%$ or $0\%$) or very small/large ($>97\%$ or $<3\%$). We end up in $22$ ``valid'' experiments with different \{V,H\} pairs, which we consider in our analysis (Table~\ref{tab:valid-experiments}).

\begin{table}[h]
\centering
\caption{Hijacking experiments with the PEERING testbed; site pairs in \{rows, columns\} correspond to \{V,H\} pairs, and ``valid'' experiments depicted with \y.}
\label{tab:valid-experiments}
\begin{tabular}{c|cccccc}
{}   & AMS & UFMG & UW & GRN & SEA & CLE\\
\hline
AMS  & { -}& {\y} &{\y}& {\y}& {\y}& {\n}\\ 
UFMG & {\y}& { -} &{\y}& {\y}& {\y}& {\n}\\
UW   & {\y}& {\y} &{ -}& {\y}& {\y}& {\n}\\
GRN  & {\y}& {\y} &{\y}& { -}& {\y}& {\n}\\
SEA  & {\y}& {\y} &{\y}& {\y}& { -}& {\y}\\
CLE  & {\n}& {\n} &{\n}& {\n}& {\y}& { -}\\
\end{tabular}
\end{table}






\pavlos{to remember: estimation accuracy vs. time from hijack (and could compare also with: nb of monitors seen the hijack vs. time from hijack) - this could be entitled as the ``real-timeness of impact estimation''}



==> experiments_setup_backup_15Jan2020.tex <==

\vkotronis{Also need to explain how we do smart IP-to-AS mapping. We apply the same practice as with the TLS scan paper, in particular:\\
We consider information that is available from the RIPE RIS~\cite{ripe2019ris} (via the RIPEstat API~\cite{ripestat2019}) and RouteViews~\cite{oregon2019rv} (via CAIDA's \texttt{pfx2as}~\cite{caida2019pfx2as}) projects, which employ globally distributed sets of Remote Route Collectors (RRCs) to collect and store Internet routing data, such as BGP updates and Routing Information Bases (RIBs). These datasets essentially map IP prefixes announced in BGP to the ASN that originates them (can be several ASNs in MOAS scenarios). We consider only non-reserved IP prefixes~\cite{wikipedia2019reservedips} and ASNs~\cite{wikipedia2019reservedasns}, that are allowed to appear in the public Internet and in BGP. Since some of the information seen in BGP might be ``tainted'', e.g., due to BGP hijack~\cite{sermpezis2018artemis} or route leak~\cite{siddiqui2014route} incidents, we apply a pre-filtering stage before using the mappings for a given date. Specifically, we consider several snapshots spanning a certain time period (e.g., the month containing the date), and within this period we preserve only the mappings that appeared consistently for more than 50\% of the total time (e.g., more than 2 weeks). This effectively filters out transient wrongful originations of certain prefixes, as observed e.g, in the case of BGP hijacks\footnote{Less than 2\% of them lasts longer than a week according to~\cite{vervier2015mind}.}. After applying this filtering stage for each per-month aggregated dataset (for RIPE RIS and RouteViews, respectively), we merge the two dataset sources by considering the union of ASNs observed per announced prefix. This results in a coverage of \todo{XXX}\% of the publicly routable IPv4 address space, on average, and provides a reasonably complete and accurate picture of IP-to-AS mappings, as seen in BGP.
}

\subsection{Data-plane Setup}

\subsubsection{Traceroutes}
We employ traceroutes from RIPE Atlas probes towards the MOAS prefix.
We extract the unique upstreams of each MOAS site and use them to differentiate which AS routes to which site; this needs to be done since after traceroute traffic entres the PEERING testbed, we cannot disambiguate the ingress point. To achieve this, we perform IP-to-AS mapping on the executed traceroutes and extract the AS of the penultimate hop before the traceroute reply enters the PEERING AS (i.e., the AS of its upstream). If we observe the following AS-level paths on probes in $ASX$ and $ASW$:
$[ASX, \dots, PEERING\_UPSTREAM\_1, PEERING\_AS, \dots]$, and\\
$[ASW, \dots, PEERING\_UPSTREAM\_2, PEERING\_AS, \dots]$\\
knowing that $PEERING\_UPSTREAM\_i$ is the unique upstream of anycast site $i, i=1,2$, then we can determine that $ASX$ is in the catchment of site $1$, while $ASW$ is in the catchment of $2$.


\subsubsection{Pings}

We employ ICMP pings issued by a PEERING client (i.e., our local machine) towards ASes in the public Internet\footnote{Note that our local client established VPN tunnels with the PEERING routers; these tunnels can be used both to issue commands on the routers on the control plane (such as ``announce this prefix over this site'' and to send packets on the data plane (such as ``IP packet from PEERING prefix to public IP'').}. We execute the following steps:

\myitem{1. Collect pingable IPs per public AS.} To achieve this, we utilize:
    \begin{enumerate}
    \item \texttt{pfx2as}: This dataset contains the Routeviews Prefix-to-AS mappings~\cite{caidapfx2as} for IPv4 and IPv6 from CAIDA, in order to map given IP prefixes (and addresses) to the ASNs that announce them in BGP. We further leverage the Pytricia prefix tree~\cite{pytricia} for longest prefix matching and fast IP address lookups. \vkotronis{need to point to the methodology paragraph on this, we use more than CAIDA's pfx2as.}
    
    \item IP hitlists from ANT Lab~\cite{antlabhitlists}: These are lists of IP addresses in the Internet that are believed to be reachable via \texttt{ping}, based on past measurements. We select only the IP addresses for which their pingability is believed with more than 90\% confidence score. By combining this information with the \texttt{pfx2as} dataset we can find pingable IPs per ASN.
    \end{enumerate}

\myitem{2. Send customized ping packets via PEERING.} For each --theoretically-- pingable IP in an ASN, we send an ICMP echo request packet out of one of the PEERING-facing tunnel interfaces of our local client. We use a source address within the prefix that we are assigned to (e.g., the first available IP address of the network), destined~to the pingable IP of the ASN, and~send it via a randomly chosen PEERING data-plane gateway towards the Internet. Custom packets are generated/crafted using the \texttt{scapy}~\cite{scapy} utility.

\myitem{3. Monitor replies via PEERING.} In case an ICMP echo reply packet comes back by re-entering PEERING and reaching our client, we monitor out of which ingress PEERING-facing tunnel interface the client received it. Resolving this interface to the corresponding MOAS site, we can determine which site attracted the traffic from the pinged AS. This methodology is similar to Verfploeter~\cite{de2017broad}, which focuses though on catchment measurement of a large CDN.
This workflow enables us to accurately measure the data-plane catchment of the deployed MOAS sites, on the AS-level.

\subsection{Control-plane Setup}

We employ CAIDA's BGPStream tool~\cite{caidabgpstream} in order to collect BGP updates related to the anycasted prefix, that were received by RouteViews and RIPE RIS monitors around the time of the experiment. We re-construct the BGP RIBs of the monitors incrementally using the observed updates, until convergence is achieved. Having the relevant --stable-- BGP AS-paths at our disposal, we extract the origin ASNs and use them to differentiate which AS routes to which site. For example, if we observe the following RIB paths on monitors $ASX$ and $ASW$:\\
$[ASX, ASY, \dots, PEERING\_AS, EXP\_ORIGIN\_1]$, and\\
$[ASW, ASZ, \dots, PEERING\_AS, EXP\_ORIGIN\_2]$\\
knowing that $EXP\_ORIGIN\_i$ is the unique experimental origin ASN of MOAS site $i, i=1,2$, then we can determine that $ASX, ASY$ are in the catchment of site $1$, while $ASW, ASZ$ are in the cathment of $2$.


==> preliminaries_backup_26Jan2020.tex <==
\subsection{Definitions: Quantities and Metrics}

We define some basic terms and metrics we use in the paper.


\myitemitnospace{Infected AS:} An AS is infected when it routes its traffic to or through the hijacker's AS.%An AS is infected when it has selected as its best path, an AS-path that contains the hijacker's ASN.

\myitemitnospace{Hijack impact}: the fraction of ASes that are \textit{infected}.

\myitemitnospace{Monitor}: an AS which can be known if it is \textit{infected} or not.

\myitemitnospace{Impact estimator:} a methodology that uses a set of \textit{monitors} and provides an estimation of the \textit{hijack impact}.

% We define the main quantities and metrics we use for the impact estimation.

% \begin{definition}[Infected AS]\label{def:infected-as}
% An AS is infected when it has selected as its best path, an AS-path that contains the hijacker's ASN.
% \end{definition}

% \begin{definition}[Hijack impact]\label{def:hijack-impact}
% The impact of a hijack is the fraction of ASes that are infected.
% \end{definition}

% \begin{definition}
% ``Monitor'' is an AS for which it can be known whether it is infected or not.
% \end{definition}


Let $I$ be the actual impact of a hijack, and an estimator $\mathcal{E}$ whose estimation is $\hat{I}_{\mathcal{E}}$. The main metrics to characterize the performance of an estimator is the \textit{bias} and the \textit{root mean square error (RMSE)}. The bias quantifies how far the expected value of the estimator is from the actual value, i.e., 
\begin{equation}
Bias_{\mathcal{E}} = E[\hat{I}_{\mathcal{E}}-I]
\end{equation}
and the RMSE quantifies the accuracy of the estimator:
\begin{equation}
RMSE_{\mathcal{E}} = \sqrt{E[(\hat{I}_{\mathcal{E}} - I)^2]}
\end{equation}
The desired characteristics for an estimator is to be \textit{unbiased} (zero bias) and have low RMSE.




\subsection{Threat Model: Hijack Types and Impact Characteristics}
We consider an AS that owns and announces a prefix $IP_{*}$ in the Internet through BGP; we denote this AS as $AS_{V}$ and call it ``victim AS''. For the sake of presentation, let the prefix $IP_{*}$ be the $10.0.0.0/8$. Every AS learns from its neighbor ASes paths to $IP_{*}$ and selects one of them as its best path; we denote the best path for an $AS_{X}$ as in the following example
\[ [AS_{X}, AS_{Y}, ..., AS_{V} | IP_{*}] \]
where $AS_{X}$ has learned this path through its neighbor $AS_{Y}$.

A hijack takes place when another AS announces an illegitimate path for the prefix $IP_{*}$, or a more specific prefix of $IP_{*}$. This is the ``hijacker AS'' and we denote it as $AS_{H}$. The hijacker's announcement may propagate to the Internet and ``infect'' some ASes (as defined above); the extent of the infection is the hijack impact.

There are different ways to perform a hijack and their impact may vary. We adopt the taxonomy used in~\cite{sermpezis2018artemis}\pavlos{I think a couple of other works used this, maybe cite them.}, and discuss their characteristics focusing on the impact.

\myitem{Origin-AS (Type-0) or Fake-path (Type-N, $N\geq1$) hijack.} In the \textit{origin-AS} hijack the $AS_{H}$ originates the $IP_{*}$ as its own, while in the \textit{fake-path} case the $AS_{H}$ announces a fake path to the $IP_{*}$ to its neighbors. The number $N$ denotes that the hijacker's ASN appears in the $N^{th}$ hop away from the origin AS. The best path of an infected $AS_{X}$ will be as in the following examples

\begin{tabular}{cl}
Type-0: &  $[AS_{X}, AS_{Y}, ..., \mathbf{AS_{H}} | IP_{*}]$\\
Type-1: &  $[AS_{X}, AS_{Y}, ..., \mathbf{AS_{H}}, AS_{V} | IP_{*}]$\\
Type-2: &  $[AS_{X}, AS_{Y}, ..., \mathbf{AS_{H}}, AS_{Z},AS_{V} | IP_{*}]$\\
Type-N: &  $[AS_{X}, AS_{Y}, ..., \mathbf{AS_{H}}, AS_{Z},..., AS_{V} | IP_{*}]$\\
\end{tabular}\\
where the link $AS_{H}-AS_{V}$ (in the Type-1 case) and the link  $AS_{H}-AS_{Z}$ (in the Type-N, $N\geq 2$,) are fake / do not exist. 

\textit{Impact characteristics:} In the Type-0 case, an AS that learns two paths, one to the victim and one to the hijacker, selects one of them as its best path based on its routing policies (e.g., preferred neighbor) and path lengths (in AS hops). In the Type-N case, since the hijacker originates a longer path than in the Type-0 case (i.e., containing N extra hops), the paths to the hijacker will appear longer and will be less preferred by some ASes, thus resulting in a lower hijack impact~\cite{sermpezis2018artemis,Jumpstarting-BGP-sigcomm-2016}. Note that the above holds in the case that no proactive measures, such as RPKI, are deployed (less than 20\% of the prefixes are currently covered by RPKI~\cite{rpki-monitor-2019,chung2019rpki}); for prefixes with RPKI, the impact decreases in Type-0 attacks due to route origin validation~\cite{reuter2018towards}, while the impact of Type-N hijacks is not affected since RPKI cannot detect fake links.

\myitem{Exact prefix or Sub-prefix hijack.} In the above examples, the The hijacker can perform a Type-0 or Type-N hijack for the same prefix $IP_{*}$ announced by the victim (\textit{exact prefix}) or for a more specific prefix in $IP_{*}$ (\textit{sub-prefix}); for example, let the $IP_{*}$ be the prefix $10.0.0.0/8$, then a sub-prefix hijack takes place if the hijacker announces the prefix $10.0.0.0/9$ (or any $10.0.0.0/d$ with $d\geq9$).

\textit{Impact characteristics:} Default routing in BGP prefers paths to more specific prefixes~\cite{ciscobestpath}. Hence, the impact of a sub-prefix hijack will be larger than an exact prefix hijack; in fact, a sub-prefix hijack will infect the entire Internet (i.e., impact 100\%) unless any proactive or filtering mechanism is applied. 

\myitem{Data-plane traffic manipulation.} Irrespectively of how the hijack is performed (Type and affected prefix), the hijacker can manipulate the traffic that attracts (from the infected ASes) in different ways, by: (i) dropping it (\textit{blackholing}), (ii) impersonating the legitimate service (\textit{imposture}), or (iii) manipulating and/or eavesdropping it and then forwarding it to the victim (\textit{man in the middle - MitM}).

\textit{Impact characteristics:} While the way the data-plane traffic is manipulated by the hijacker does not affect the impact on the control plane (i.e., as defined in this paper), it determines which hijack detection mechanisms that can be applied (cf. data-plane vs control-plane approaches, Section~\ref{}), as well as the applicable impact estimation mechanisms, which we discuss later in the paper. In particular, mechanisms using ping measurements may not be applicable in MitM hijacks, since a ping packet will be forwarded from the hijacker to the victim.



\subsection{Hijack Datasets and Simulation Methodology}%Simulation Methodology
To study, evaluate, and compare different impact estimation approaches, we would need ground truth data about hijack events containing details, such as, victim and hijacker ASes, hijack type, set of ASes that are infected, etc. However, typically the details of hijacking events are not publicly reported, and a detailed dataset does not exist, to our best knowledge\footnote{The BGPmon service~\cite{commercial-bgpmon}, which was suspended in 2019, reported about potential hijacking events, but without providing the detailed information we would need. While there are ongoing research activities on building a database of hijacking events~\cite{caida-observatory}, no public datasets are made available yet.}. Therefore, we use realistic simulations to compile detailed datasets of hijacking events.


Specifically, we simulate the Internet routing system using a largely adopted methodology~\cite{ballani2007study,Let-the-market-BGP-sigcomm-2011,how-secure-goldberg-ComNet-2014,Jumpstarting-BGP-sigcomm-2016,RPKI-deployment-2016,sermpezis2019pomacs, sermpezis2018artemis}: (i) we use the CAIDA's AS-relationship dataset~\cite{AS-relationships-dataset} that contains AS-links and inferred inter-AS economic relationships (\textit{customer to provider}, \textit{peer to peer}), based on which (ii) we build the Internet topology graph representing each AS as a single node (a reasonable assumption for the vast majority of ASes~\cite{muhlbauer2006building}) and (iii) we define the routing policies of each AS as in the classic Gao-Rexford conditions~\cite{stable-internet-routing-TON-2001}, where an AS prefers routes to a prefix learned from its customers, then its peers, and then its providers (due to lack of more fine grained information, local preferences for neighbors of the same type are randomly set), and then (iii) we simulate BGP message exchanges between connected ASes using the simulator of~\cite{sermpezis2019pomacs}. For each hijack type, we simulate $1000$ scenarios with different \{victim, hijacker\} pairs.


% Specifically, we use a BGP simulator, based on the AS-relationships dataset~\cite{AS-relationships-dataset} (containing customer-provider and peer-peer relationships) and \vkotronis{assume policies in accordance with the} valley-free routing model. Specifically, in the simulations, each AS is represented as a single node, and first prefers routes to a prefix learned from customers, then from peers, and then from providers. Among multiple routes learned from the same type of neighbors, the AS prefers the shortest, and if more than one exist, then it prefers the route from the neighbor of the highest local preference; due to lack of information, local preferences for neighbors of the same type are randomly set for each AS.

% \vkotronis{Shouldn't we refer here to the SIGMETROCS paper model and methodology? Also we need to make clear that we map an anycast catchment inference methodology to hijack impact inference by considering the hijacker as an illegitimate ingress point/PoP.}


While, admittedly, simulations based on the AS-relationships dataset and valley-free routing model may not generate the exact impact output per \{V,H\} case, they have been shown to capture well the routing decisions for the majority of ASes~\cite{routing-policies-in-the-wild,sermpezis2019pomacs}. In our study, we focus on the statistical characteristics of the impact estimation rather than on the per case behavior, and thus the impact of uncertainty or randomness is not expected to be significant. \red{Moreover, in Section~\ref{sec:real-world-exp} we conduct real hijacking experiments on the Internet, apply our methods in the wild, and validate them with real data.}



\subsection{Measurement Tools and Services}\label{sec:preliminary-measurements}

In the paper we use control and data plane measurement data from a set of publicly available monitors:%, namely, route collectors (RC) and probes from RIPE Atlas (RA):

\myitem{Route collectors (RC)}: The RIPE RIS~\cite{riperis} and RouteViews~\cite{routeviews} projects provide BGP RIBs and updates collected from several hundred of ASes %more than 400 ASes 
worldwide. We refer to these ASes that peer with the RIPE RIS and RouteViews route collectors and provide their BGP feeds as ``route collector monitors'', or for brevity ``RC''; in the paper, we consider a set of 228 RC that consistently provided data in our experiments (see Section~\ref{sec:real-world-exp}). The RC enable \textit{control-plane monitoring}, since they provide a feed of the BGP updates (best paths exported to route collectors).  

\myitem{RIPE Atlas probes (RA)}: 
The RIPE Atlas~\cite{ripeatlas} platform comprises more than $25k$ probes (in $\sim3.5k$ ASes), \ie devices able to run pings and traceroutes towards certain Internet destinations. We refer to the set of ASes with at least one RIPE Atlas probe as ``RA'' monitors, which in our experiments account for 3420 ASes. The RA enable \textit{data-plane monitoring}, when conducting from the probes traceroutes that return the IP-path to the prefix.

\vkotronis{@pavlos: could you update the related numbers by looking at the ``best'' experiments in PEERING results? You can check the numbers in the AMS experiments}

\vkotronis{Should we mention the ping methodology here or does this section contain only public available services?}



==> temp.tex <==
\subsection{Secondary metrics}

\textit{Remark:} Other secondary metrics for the estimator accuracy we refer to in the paper are the \textit{mean absolute error (MAE)} and the \textit{relative MAE error (RelMAE)}
\begin{align}
MAE_{\mathcal{E}} &= E[|\hat{I}_{\mathcal{E}} - I|]\\
RelMAE_{\mathcal{E}} &= E\left[\frac{|\hat{I}_{\mathcal{E}} - I|}{I}\right]
\end{align}
\begin{proposition}\label{thm:rmse-vs-mae}
For any estimator $\mathcal{E}$, it holds: $RMSE_{\mathcal{E}}\geq MAE_{\mathcal{E}}$
\end{proposition}
\begin{proof}
Appendix~\ref{appendix:proof-rmse-vs-mae}
\end{proof}

\vkotronis{You can also apply Cauchy-Schwarz inequality (\url{https://math.stackexchange.com/questions/687509/using-cauchy-schwarz-inequality-to-prove-that-the-mean-of-n-real-numbers-is-less})}


\subsection{Impact Estimation: The Naive Measurement-based Method}


We also consider the sets \textbf{RC+} and \textbf{RA+}, in which we augment the set of monitors with the set of ASes seen in the monitors' paths\footnote{For example, let assume a single RC monitor $AS_{x}$, which has a path $[AS_{x}, AS_{y}, AS_{z}, origin~AS]$; then \textbf{RC} = \{$AS_{x}$\} and \textbf{RC+} = \{$AS_{x},AS_{y},AS_{z}$\}.}. 

The average number of monitors are given in Table~\ref{tab:nb-monitors}. There are an order of magnitude more data-plane monitors (RA) than control-plane monitors (RC), and augmenting the sets leads to 13\% (RA+) and 18\% (RC+) more monitors, respectively.
% \begin{table}[h]
% \caption{Avg \#ASes in monitor sets.}
% \label{tab:nb-monitors}
% \centering
% \begin{tabular}{l|cc}
% {}   &  {RC (RC+)} & {RA (RA+)}\\
% \hline
% {Avg \#ASes} &  {228 (270)} &   {3420 (3860)}
% \end{tabular}
% \end{table}

\question{Does the ``naive'' method accurately estimate the hijack impact?}

A quick answer is ``No'', or ``Not much'', or even ``It depends'': on average, the relative errors are more than 20\%, which in absolute error this corresponds to around 8\%. 


Table~\ref{tab:avg-error} gives the average relative error in the impact estimation with the ``naive'' method,  calculated as
\[
\textstyle \text{relative error} = \frac{\left| \text{impact estimation} - \text{real impact}\right|}{\text{real impact}}
\]
as well as the absolute errors calculated as
\[
\textstyle \text{absolute error} = \left| \text{impact estimation} - \text{real impact}\right|
\]

\begin{table}[h]
\centering
\caption{Average errors of ``naive'' impact estimation. \\
(the avg. real impacts for Types-\{0,1,2\} are \{0.5, 0.3, 0.19\})}
\label{tab:avg-error}

\begin{tabular}{l|ccc}
\multicolumn{4}{c}{\textbf{Relative error}}\\
{}   &  {Type-0}     &   {Type-1}    & {Type-2}\\
\hline
{RC}        &  {0.26}   &   {0.56}  & {0.59}\\
{RA}        &  {0.22}   &   {0.33}  & {0.39}
\end{tabular}
\begin{tabular}{l|ccc}
\multicolumn{4}{c}{\textbf{Absolute error}}\\
{}   &  {Type-0}     &   {Type-1}    & {Type-2}\\
\hline
{RC}        &  {0.08}   &   {0.07}  & {0.05}\\
{RA}        &  {0.07}   &   {0.06}  & {0.04}
\end{tabular}
\end{table}

The relative error is always larger than 20\%, and increases with the hijack type. RA achieves lower error than RA \vkotronis{@PS: you mean ``than RC'' right?}. The results are similar when considering the sets RC+ and RA+ (for detailed results see Appendix~\ref{appendix:naive-method}). When it comes to the absolute error, the average values are between 4\%-8\%; depending on the use case, these errors may be acceptable, however, the average real impact of a hijack needs to be taken into account (e.g., while the avg impact estimation error for Type2 hijack is only 4\%, this corresponds to an average real impact of 19\%, i.e., $\frac{4\%}{19\%}\approx \frac{1}{4}$).

Moreover, we present the distribution of the relative error in Fig.~\ref{fig:sims-impact-rc-vs-hijack-types} for the RC case (the RA case is similar, see Appendix~\ref{appendix:naive-method}). As can be seen, in 40\% of the cases for hijack Type-0 (red line, $y=0.6$), the error is larger than 20\% ($x=0.2$). The CDF for the absolute error is given in Fig.~\ref{fig:sims-impact-rc-vs-hijack-types-abs-error}.



\begin{figure}
\centering
\subfigure[relative error]{\includegraphics[width=0.49\linewidth]{./figures/fig_impact_RC_vs_hijackTypes.eps}\label{fig:sims-impact-rc-vs-hijack-types}}
\caption{CDF of the (a) relative and (b) absolute error of impact estimated by the ``naive'' method with measurements from route collectors (RC) for hijacks of Types-0, 1, and 2.}
\label{fig:sims-impact-cdf-naive-relative-absolute-errors}
\end{figure}






\subsection{Next steps}
\question{How to improve the accuracy of the naive method?}

\question{Can a (only) measurement-based method achieve high accuracy?}

\question{How robust is the impact estimation wrt. the number of monitors?} 
\pavlos{TODO: Select (randomly?) a subset of the monitors, and calculate the impact only based on them. Plot avg error vs. \# of monitors in the subset.}

\myitem{Idea [R-graph]:} An R-graph assisted measurement method could exploit the information about AS-relationships and achieve higher accuracy. An initial investigation of this, follows, in Section~\ref{sec:impact-estimation-Rgraph}.

\myitem{Idea [collectors similarity]:} The bias in the impact estimation may be due to the fact that monitors are not uniformly located in the Internet topology, and thus not representative of the entire Internet routing system. For sets of monitors that are very similar, keep only one of them. For an initial investigation, see Section~\ref{sec:monitor-similarity}.



\subsection{Impact Estimation: The R-graph based method}\label{sec:impact-estimation-Rgraph}
\myitem{R-graph based impact estimation (``R-graph''):} Estimate the hijack impact, by building the R-graph~\cite{sermpezis2019pomacs} for the hijacker and victim ASes and inferring the catchment of the hijacker.

Two estimators can be used:
\begin{itemize}[leftmargin=*]
    \item \textbf{Certain catchment}: the fraction of infected ASes among the ASes with a certain inference: 
    \[\frac{\text{\# infected ASes with certain inference}}{\text{\# ASes with certain inference}}\]
    \item \textbf{Probabilistic catchment}: the sum of the ASes probabilities to route to the hijacker over the total number of ASes: 
    \[\frac{\sum_{AS} Prob\{AS\rightarrow Hijacker\}}{\text{\#ASes}}\]
\end{itemize}
Moreover, the certain/probabilistic inference can be enhanced by measurements (with RC and/or RA).

Table~\ref{tab:avg-error-Rgraph} gives the average relative ans abolute error in the impact estimation with the ``R-graph'' method for hijacks of Type-0. The results show that taking into account the routing and AS-relationship information can significantly improve the accuracy of impact estimation, compared to the ``naive'' approach. The estimator based on the probabilistic inference is more accurate than the certain inference (which takes into account only a subset of ASes); more results comparing these two estimators can be found in Appendix~\ref{appendix:Rgraph-method}.

\begin{table}[h]
\caption{Average errors of ``R-graph'' impact estimation for hijack Type-0. \pavlos{TODO: run more sims for stat confidence.}}
\label{tab:avg-error-Rgraph}
\centering
\begin{tabular}{l|ccc}
\multicolumn{4}{c}{\textbf{Relative error}}\\
{}   &  {no measurements}     &   {with RC}    & {with RA}\\
\hline
{certain}        &  {0.14}   &   {0.10}  & {0.07}\\
{probabilistic}  &  {0.09}   &   {0.05}  & {0.04}
\end{tabular}
\begin{tabular}{l|ccc}
\multicolumn{4}{c}{\textbf{Absolute error}}\\
{}   &  {no measurements}     &   {with RC}    & {with RA}\\
\hline
{certain}        &  {0.05}   &   {0.03}  & {0.02}\\
{probabilistic}  &  {0.03}   &   {0.02}  & {0.01}
\end{tabular}
\end{table}

Moreover, Fig.~\ref{fig:sims-impact-Rgraph-prob} shows the distribution of the relative error for the ``R-graph'' method using the (more accurate) probabilistic inference estimator, for three cases where no measurements, measurements with RCs, and measurements with RAs are used. The improvement by using RC and RA is similar; in almost 80\% of the cases (y-axis), the error is less than 5\% (x-axis), and almost always the error is less than 20\%.

\myitem{Main insight [``R-graph'' as an upper bound for accuracy]:} The ``R-graph'' method shows the improvement by taking into account the available information about routing policies. Under a ``perfect'' environment, where our knowledge about the routing policies is accurate (i.e., no AS-links are missing, routing is valley free, and no AS-relationships are mis-inferred) , the ``R-graph'' gives an upper bound for the accuracy we can achieve in impact estimation.

\question{The accuracy of the ``R-graph'' method is superior; can we (and how to) exploit the R-graph to improve a measurement-based method (e.g., selection of monitors)?}\pavlos{Working on this...}

\vkotronis{I do not fully agree with this remark. It is superior in simulations, which also assume exactly the same setup as the R-graph; however in the wild we do not know what happens if e.g., a subset of ASes follow different policies. Comparing the R-graph with the simulated impact under exactly the same known policy assumptions might be biased. However, I agree that the monitors have worse performance, but I do not know how worse if we do not take into account the biases of the VF assumptions (and others, like single-node ASes etc.). What do you think?}


\begin{figure}
\centering
\subfigure[relative error]{\includegraphics[width=0.49\linewidth]{./figures/fig_impact_Rgraph_prob_hijackType0.eps}\label{fig:sims-impact-Rgraph-prob}}
\subfigure[absolute error]{\includegraphics[width=0.49\linewidth]{./figures/fig_impact_Rgraph_prob_hijackType0_absError.eps}\label{fig:sims-impact-Rgraph-prob-absolute-error}}
\caption{CDF of the (a) relative and (b) absolute error of impact estimated by the ``R-graph'' method with probabilistic inference enhanced by no measurements, measurements by RC, and measurements by RA. }
\label{fig:sims-impact-cdf-Rgraph-relative-and-absolute-errors}
\end{figure}


\subsection{Monitor Similarity and Impact Estimation}\label{sec:monitor-similarity}

We now investigate whether there is some similarity between monitors, and if it affects the impact estimation. 

\myitem{Key finding:} (spoiler :) ) There is no strong relation between monitor similarity and impact estimation.


We first define the following measures of similarity, which are based only on routing information.
\begin{itemize}[leftmargin=*]
    \item \textbf{Jaccard similarity:} Let two monitors $X$ and $Y$, and let $P_{X}$ (and $P_{Y}$) be the set of ASNs seen in the AS-path by the monitor $X$ (and $Y$). Then the Jaccard index/similarity is 
    \[S_{X,Y} = \frac{|P_{X} \cap P_{Y}|}{|P_{X} \cup P_{Y}|}\]
    A similar metric of similarity, based on seen routing paths and the Jaccard index has been used in~\cite{holterbach2017measurement} for selecting vantage points for measurements (mainly for RIPE Atlas probes).\footnote{We considered also other similar measures, such as $\frac{|P_{X} \cap P_{Y}|}{min \{|P_{X}|, |P_{Y}|\}}$ or $\frac{|P_{X} \cap P_{Y}|}{|P_{X}|}$, but the initial findings were very close to the Jaccard similarity measure. We could do a deeper investigation if needed later.}

    \item \textbf{R-graph similarity:} Let $C_{X}$ be the set of ASes that can be reached by following directed edges in the R-graph from the monitor $X$; in other words, $C_{X}$ is the ``catchment'' of X, or the set of nodes whose paths to the victim/hijacker may contain the monitor $X$. Then, the R-graph similarity is defined as:
    \[S_{X,Y} = \frac{|C_{X} \cap C_{Y}|}{|C_{X} \cup C_{Y}|}\]
\end{itemize}

\textit{Remark:} (a) The Jaccard similarity measure, takes into account the ASes \textit{before the monitor}, i.e., the ASes between the victim (or hijacker) and the monitor; two monitors with Jaccard similarity 1, will have common path to the victim (or hijacker). On the contrary, the R-graph similarity measure takes into account the ASes \textit{after the monitor}; two monitors with R-graph similarity 1, will affect the same set of ASes. (b)  The Jaccard similarity measure can be calculated only from measurements, while the R-graph similarity can be calculated only from simulations (however, mix of sims-measurements can be used in both measures).

The average similarity between monitors calculated in simulations, were 0.39 (RC) and 0.33 (RA)  for the Jaccard measure, and negligible for the R-graph measure. 

Moreover, the correlation between the average monitor similarity in a simulation run with the impact estimation error is given in Table~\ref{tab:monitor-similarity}, where we can see that there is no strong correlation (for more detailed results, see Appendix~\ref{appendix:monitor-similarity}).


\begin{table}[h]
\centering\caption{Correlation (Pearson's coefficient) between average monitor similarity and impact estimation error.}
\label{tab:monitor-similarity}
\begin{tabular}{c|rr}
{} & {Jaccard} & {R-graph}  \\
\hline
{RC} & {~0.09} & {~0.02} \\
{RA} & {~0.21} & {-0.08} \\
\end{tabular}
\end{table}

Summarizing, probably these similarity measures cannot be exploited to improve the impact estimation (e.g., by removing similar monitors, or selecting dissimilar ones \pavlos{some initial tests I did with heuristics for monitor selection based on similarity indicated this as well, i.e., they did not improve accuracy}).

\question{Are there other measures or other information (i.e., not only routing paths) that could be used? Would/Could the main findings remain the same or change significantly?}




\subsection{Impact Estimation: ML models}\label{sec:impact-estimation-ML}
\pavlos{tentative results in Tables~\ref{tab:LinR-w-vs-nbMons} and~\ref{tab:LinR-w-vs-hijackType}, and Figures~\ref{fig:ML-2D-visualization-Impact-closeness} and~\ref{fig:MAE-vs-nb-monitors}}

\myitem{Linear Regression model.}
\begin{align*}
\hat{I} &= w_{2}\cdot NIE + w_{1}\cdot closeness + w_{0} \\
        &= w_{2}\cdot \frac{1}{M}\displaystyle\sum_{i\in\mathcal{M}}m_{i} + w_{1}\cdot \frac{1}{M}\displaystyle\sum_{i\in\mathcal{M}}\mathbb{I}_{dV_{i}>dH_{i}}-\mathbb{I}_{dH_{i}>dV_{i}}+ w_{0}
\end{align*}


% \begin{table}[h]
% \centering
% \caption{Weights of the features in the Linear Regression model for impact estimation vs. number of measurements.}
% \label{tab:LinR-w-vs-nbMons}
% \begin{tabular}{l|ccccccc}
% {}          & \multicolumn{7}{c}{\#monitors (M)}\\
% Features    & {229}& {100}& {50}& {30}& {20}& {10}& {5} \\
% \hline
% NIE         & { 0.88}& { 0.88}& { 0.84}& { 0.84}& { 0.79}& { 0.76}& { 0.67} \\
% closeness   & {-0.09}& {-0.09}& {-0.09}& {-0.10}& {-0.07}& {-0.07}& {-0.05} \\
% 1           & { 0.10}& { 0.11}& { 0.13}& { 0.123}& { 0.15}& { 0.16}& { 0.19}
% \end{tabular}
% \end{table}


% \begin{table}[h]
% \centering
% \caption{Weights of the features in the Linear Regression model for impact estimation vs. type of hijack (for measurements with all 229 RC monitors).}
% \label{tab:LinR-w-vs-hijackType}
% \begin{tabular}{l|ccccccc}
% {}          & \multicolumn{3}{c}{Hijack Type}\\
% Features    & {0}& {1}& {2}\\
% \hline
% NIE         & { 0.88}& { 0.79}& { 0.74} \\
% closeness   & {-0.09}& { 0.01}& { 0.04}\\
% 1           & { 0.10}& { 0.04}& { 0.02}
% \end{tabular}
% \end{table}





\begin{figure}
\centering
\subfigure[Hijack Type-0]{\includegraphics[width=0.49\linewidth]{./figures/fig_ML_MAE_vs_nbMons_hijack_type0.eps}\label{fig:MAE-vs-nb-monitors-type0}}
\caption{MAE (y-axis) of naive impact estimator (NIE) and ML-based linear regression estimator (LinR) vs. number of nodes measured (x-axis); comparison with R-graph estimator as reference.}
\label{fig:MAE-vs-nb-monitors}
\end{figure}




\begin{table}[h]
\centering
\caption{Linear Regression models \pavlos{to be removed}}
\label{tab:my_label}
\begin{tabular}{c|c|ccc}
{}   & {}      & \multicolumn{3}{c}{Model parameters}\\
Estimator   & RMSE      &   $w_{0}$ & $w_{NIE}$ & $w_{feature}$\\
\hline
NIE         & 10.0\%     &-&-&-\\
LRE(AS-rel) & 7.9\%     & 0.04 & 0.92 & 0.11\\
LRE(dist)   & 7.4\%     & 0.12 & 0.77 & -0.08\\
LRE(vf)   & 8.3\%     & 0.12 & 0.77 & -0.08\\
\end{tabular}
\end{table}




\begin{table*}[h]
%\centering
\caption{Model parameters of LRE vs. number of monitors (for hijack Type-0) and vs. hijack types (for all RC monitors).}
\label{tab:LRE-parameters-vs-nbMons}
\begin{tabular}{cl|cccccc||ccc}
{}&{}          & \multicolumn{6}{c}{\#monitors (M)}& \multicolumn{3}{c}{Hijack Type}\\
\multicolumn{2}{c|}{Parameters}    & {229}& {100}& {50}& {20}& {10}& {5} 
    & {0}& {1}& {2}\\
\hline
\multirow{3}{*}{\shortstack{LRE\\($f_{pref}$)}}
&$w_{0}$   & {0.04}& {0.04}& {0.06}& {0.09}& {0.14}& { 0.19}
    & {0.04}& {0.02}& {0.01}\\
&$w_{NIE}$ & {0.92}& {0.91}& {0.88}& {0.81}& {0.73}& { 0.63} 
    & {0.92}& {0.84}& {0.81}\\
&$w_{f}$   & {0.11}& {0.11}& {0.10}& {0.06}& {0.03}& { 0.04}
    & {0.11}& {0.05}& {0.01}\\
\hline
\multirow{3}{*}{\shortstack{LRE\\($f_{dist}$)}}
&$w_{0}$  & { 0.12}& { 0.12}& { 0.13}& { 0.14}& { 0.17}& { 0.22}
    & { 0.12}& { 0.04}& { 0.02}\\
&$w_{NIE}$& { 0.77}& { 0.76}& { 0.74}& { 0.72}& { 0.67}& { 0.58} 
    & { 0.77}& { 0.80}& { 0.80}\\
&$w_{f}$  & {-0.08}& {-0.08}& {-0.08}& {-0.07}& {-0.05}& {-0.05} 
    & {-0.08}& {-0.04}& { 0.00}\\
\end{tabular}
\end{table*}

==> understanding_backup_26Jan2020.tex <==
In this section, we aim to understand and characterize the  problem of hijack impact estimation using (passive and active) measurements, identify associated practical challenges, and take the first steps towards designing an estimator. 

\subsection{Measuring the Hijack Infection}
The hijack impact is determined by the number of infected ASes. Hence, the basic step for the estimation of the hijack impact is to identify whether an AS is infected or not. To this end, different types of network measurements can be employed (and have been used by the hijack detection mechanisms~\cite{}). While their detailed detection mechanisms have been extensively studied in literature and are out of the scope of this paper, we provide only some indicative examples and discuss their main characteristics in the context of the impact estimation:

\vkotronis{@pavlos: check out also Section~\ref{sec:real-world-exp}}

\myitem{Route collectors - BGP updates:} The route collectors provide control-plane information (BGP updates and RIBs) received from their peers (``monitors''). An infected monitor can be detected from the AS-path or the prefix in its BGP updates (see~\cite{sermpezis2018artemis} for a comprehensive approach); e.g., for a Type-0 hijack we check the first ASN in the path and if is different than $AS_{V}$ then the monitor is infected .


\pavlos{control-plane information, real-time, passive measurement, low overhead}

\myitem{RIPE Atlas probes - traceroutes:} Conducting a traceroute from a probe to the hijacked prefix, will provide a path of IP addresses to the destination. Mapping the IPs to ASNs, we can infer the AS-path followed, and thus detect (similarly to the BGP updated approach) whether the AS hosting the probe (i.e. ``monitor'') is infected.

\pavlos{data/control-plane information, active measurement, potential limitations/inaccuracies from mapping IP to AS, quantify overhead (time needed, RA credits per measurement)}
\vkotronis{Why control-plane too? Due to the IP-to-AS mapping, right?}

\myitem{Ping campaigns:} The victim can ping (from its network) an IP address in a remote AS; if the ping response returns to the victim's network, then the AS can be inferred as not infected (see, e.g., the relevant techniques of~\cite{de2017broad, Zhang-Ispy-CCR-2008}). However, note that this inference can be correct in blackholing and imposture hijacks, but not in MitM attacks. 

\pavlos{data-plane information, active measurement, arbitrary destinations, requires custom system/script(?), quantify overhead (time needed), limitations of finding/maintaining a list of responsive IP addresses and bias due to unresponsive addresses}


% \begin{definition}
% ``Monitor'' is an AS for which it can be known whether it is infected or not.
% \end{definition}
In the above context, a ``monitor'' can be a peer of a route collector that pushes BGP updates to the route collector, an AS that hosts one or more RIPE Atlas probes, or an AS with a responsive pingable IP address (i.e., almost every AS).

\subsection{Naive Impact Estimation (NIE)}
The most intuitive approach to estimate the impact of a hijack is to measure a number of ASes (i.e., ``monitors''), and estimate the hijack impact as the fraction of infected monitors (i.e., number of infected monitors over the total number of monitors). We refer to this approach as the \textit{Naive Impact Estimation} and formally define it as follows.

\begin{definition}[Naive Impact Estimator (NIE)]\label{def:naive-impact-estimator}
Let a set of monitors $\mathcal{M}$ ($|\mathcal{M}|=M$), and an indicator $m_{i}$ denoting whether monitor $i\in\mathcal{M}$ is infected ($m_{i}=1$) or not ($m_{i}=0$). The Naive Impact Estimator estimates the hijack impact as 
\begin{equation}
\hat{I}_{NIE(\mathcal{M})} = \frac{1}{M}\textstyle\sum_{i\in\mathcal{M}}m_{i}
\end{equation}
\end{definition}

The NIE can be used with any type of measurements (e.g., BGP messages, traceroutes, pings) that can provide information for calculating the indicator $m_{i}$. In the following we study the properties of NIE, and its accuracy when combined with different types of measurements and monitor sets.



\subsection{Accuracy of the NIE}

\mysubsubsection{1) NIE with Random Set of Monitors}

In the following theorem, we prove that, when the set of monitors $\mathcal{M}$ is randomly selected, the NIE is an \textit{unbiased estimator}, and we derive an expression for its RMSE that is a function of the number of monitors $M$ and the hijack type.

\begin{theorem}\label{thm:NIE-bias-rmse}
Under a randomly selected set of monitors $\mathcal{M}$, the bias and root mean square error of NIE are given by
\begin{equation*}
Bias_{NIE} = 0 
~\hspace{0.3cm}\text{and}\hspace{0.3cm}~ 
RMSE_{NIE} = \frac{1}{\sqrt{M}}\cdot c_{I}
\end{equation*}
where $c_{I}= \int_{0}^{1} \sqrt{I\cdot (1-I)}\cdot f(I)\cdot dI$, is a constant that depends on the impact distribution $f(I)$.
\end{theorem}
% \begin{theorem}\label{thm:NIE-bias-rmse}
% Under a randomly selected set of monitors $\mathcal{M}$, the NIE is an unbiased estimator, i.e.,  
% \begin{equation*}
% Bias_{NIE} = E[\hat{I}-I] = 0 \hspace{0.5cm} \Leftrightarrow \hspace{0.5cm} E[\hat{I}] = I
% \end{equation*}
% and its root mean square error (RMSE) is given by
% \begin{equation*}
% RMSE_{NIE} = \sqrt{E[(\hat{I} - I)^2]} = \frac{1}{\sqrt{M}}\cdot c_{I} 
% \end{equation*}
% where $c_{I}$ is a constant that depends on the impact distribution $f(I)$, and is given by
% \begin{equation*}
% c_{I} = \int_{0}^{1} \sqrt{I\cdot (1-I)}\cdot f(I)\cdot dI    
% \end{equation*}
% \end{theorem}
\begin{proof}
The detailed proof is given in Appendix~\ref{appendix:proof-NIE-bias-rmse}. Here, we only state an intermediate result in the proof to provide intuition about $c_{I}$: For a hijack with impact $I$, the RMSE of NIE is given by $RMSE_{NIE}(I) = \frac{1}{\sqrt{M}}\cdot \sqrt{I\cdot(1-I)}$. 
%
Then, $c_{I}$ is calculated by taking the expectation over all possible hijack impacts $c_{I}= \int_{0}^{1}RMSE_{NIE}(I)\cdot f(I)\cdot dI$.
\end{proof}


\textit{Remark:} The impact distribution $f(I)$ depends on the \{V,H\} pairs that are expected to be involved in a hijack and the hijack types.
%The impact distribution $f(I)$ depends on the \{V,H\} pairs, the hijack type, and the frequency (or, realization probability) of hijacks per type and per pair
For example, if any pair of ASes is equally probable to be the \{V,H\} pair, then the impact $I$ of a Type-0 hijack can be shown to be approximately uniformly distributed in $[0,1]$. In this case, the constant $c_{I}$ is $c_{I}(Type-0) = \frac{\pi}{8}\approx 0.39$. 

The following table gives the values of the hijack constant $c_{I}$ calculated experimentally among $1000$ simulation for random \{V,H\} pairs. We also consider scenarios that are closer to reported hijacking activity: namely, scenarios where (i) the \{V,H\} ASes correspond to the events identified as potential hijacks by the BGPmon service in 2018~\cite{commercial-bgpmon, arakadakis-conext2018-poster}, and (ii) hijackers are from the set of $22$ ASes classified as ``serial hijackers''~\cite{testart2019profiling} and victims are selected randomly.
\pavlos{Maybe add a plot for these cases next to Fig.~\ref{fig:RMSE-NIE-random-vs-nb-monitors}.}


\begin{table}[h]
\centering
\caption{Experimentally calculated hijack constant $c_{I}$ (in the parentheses, $E[I]$: the corresponding values for the average impact) for different hijack types and \{V,H\} pairs.}
\label{tab:hijack-constant}
\begin{tabular}{l|ccc}
   & Type-0 & Type-1 & Type-2  \\
\hline
random \{V,H\} pairs         & 0.39 (0.50) & 0.36 (0.30) & 0.31 (0.19)\\
BGPmon \{V,H\} pairs~\cite{arakadakis-conext2018-poster}         & 0.35 (0.43) & 0.29 (0.26) & 0.22 (0.17)\\
random V, ``serial'' H~\cite{testart2019profiling}  & 0.37 (0.68) & 0.40 (0.49) & 0.36 (0.31)
\end{tabular}
\end{table}

\textit{Remark:} The RMSE(I) is not equal for all values of the real impact. In fact, it is a concave function with a maximum $\frac{1}{2\cdot\sqrt{M}}$ at $I=0.5$ , and minimum $0$ at the corner cases of $I=0$ and $I=1$. In other words, it becomes more difficult to estimate with high accuracy when the victim and hijacker attract similar fractions of AS routes. This explains the lower values of $c_{I}$ for higher-$N$ hijack types: as $N$ increases, the mass of the impact distribution concentrates around smaller values --closer to $I=0$-- in the area of which the RMSE(I) takes low values.


Figure~\ref{fig:RMSE-NIE-random-vs-nb-monitors} shows the RMSE of the NIE with a random set of monitors as calculated from Theorem~\ref{thm:NIE-bias-rmse} for hijacks of Type-0, 1, and 2, where the constants $c_{I}$ are taken from Table~\ref{tab:hijack-constant}; simulation results (over 1000 simulation runs) coincide with the theoretical results and omitted from the figure.
\begin{figure}
\centering
\subfigure[NIE (random monitors)]{\includegraphics[width=0.49\linewidth]{./figures/fig_RMSE_random_vs_M.eps}\label{fig:RMSE-NIE-random-vs-nb-monitors}}
\subfigure[NIE (Type-0 hijack)]{\includegraphics[width=0.49\linewidth]{./figures/fig_RMSE_random_RC_RA_vs_M_hijack0.eps}\label{fig:RMSE-NIE-random-RC-RA-vs-nb-monitors-Type0}}
\caption{RMSE of the NIE (y-axis) vs. number of monitors (x-axis): (a) random set of monitors for hijacks of Type-0, 1, 2; (b) random sets, RC, and RA monitors for Type-0 hijacks \pavlos{maybe add here the lower bound of the Rgraph}.}
\label{fig:RMSE-NIE-vs-nb-monitors}
\end{figure}


\mysubsubsection{2) NIE with Monitors from Public Measurement Services}

We now investigate the accuracy of NIE when using the publicly available monitors RC and RA (see Section~\ref{sec:preliminary-measurements}), which are \textit{not} uniformly located in the Internet~\cite{routeviews-list-collectors,riperis-list-collectors}. 

At first, when considering all possible \{V,H\} pairs with the same probability, NIE with \textit{any} set of monitors (i.e., including the RC and RA cases) is an unbiased estimator.
\begin{corollary}\label{thm:unbiased-NIE-generic}
$Bias_{NIE(\mathcal{M})} = E[\hat{I}-I] =0,~\forall \mathcal{M}$, when the expectation is taken over all possible \{V,H\} node pairs.
\end{corollary}
\begin{proof}
Appendix~\ref{appendix:unbiased-NIE-generic}.
\end{proof}

However, the above result does not mean that the \textit{accuracy} of NIE is the same $\forall\mathcal{M}$. In fact, the accuracy heavily depends on the set of monitors. This is clearly demonstrated in Table~\ref{tab:NIE-with-public-monitors} that compares simulation results for the RMSE of the NIE using public monitors against the corresponding RMSE of the NIE with random sets of monitors; the sizes of random sets are equal to the number of the public monitors in each case.

\begin{table}[h]
\caption{RMSE for NIE with public monitors (and random set of monitors) for different hijacks types.}
\label{tab:NIE-with-public-monitors}
\centering
\begin{tabular}{l|ccc}
{}   &  {Type-0}     &   {Type-1}    & {Type-2}\\
\hline
{RC, 228 monitors}        &  {10\% (2.6\%)}   &   {~9\% (2.4\%)}  & {~8\% (2.1\%)}\\
{RA, 3420 monitors}        &  {~9\% (0.7\%)}   &   {~8\% (0.6\%)}  & {~7\% (0.5\%)}
\end{tabular}
\end{table}

\myitemit{Key finding:} \textit{The (non-uniform) locations of the public monitors heavily affect the accuracy of NIE.}

A NIE using the monitors of the public services has a RMSE of 9\%-10\% for Type-0 hijacks, while the same estimator with randomly selected monitors would achieve almost 5 times (2.6\%) and 10 times ($<1\%$) lower RMSE when the number of monitors is equal to the number of RC and RA monitors, respectively; similar results hold for all hijack types. It is interesting to observe that despite the fact that there are an order of magnitude more data-plane monitors (RA) than control-plane monitors (RC), the accuracy is very similar: RA achieves only 1\% lower RMSE than RC.

\vkotronis{We need to drill down and find a justification for the latter statement. Need to think about it, in conjunction with the deployment practices of RA, RIS and RV.}


\myitemit{Key finding:} \textit{Measuring 50 monitors of public services, is typically enough for achieving close to the(ir) highest possible accuracy with NIE.}

Figure~\ref{fig:RMSE-NIE-random-RC-RA-vs-nb-monitors-Type0} compares the RMSE of NIE with random, RC, and RA monitors for hijacks of Type-0 as a function of the number of monitors used (in the case of RC and RA, in each simulation run we select a random subset of size M). We can observe that the RMSE of NIE with RC or RA reaches the plateau of around 10\% after 30-50 monitors; for the same number of monitors, the RMSE of NIE with random monitors is two times lower (around 5\%) and further decreases with the number of monitors. Similar findings hold for the case of hijack types 1 and 2, which we omit due to space limitation. %(see Appendix~\ref{appendix:naive-method} - Fig.~\ref{fig:RMSE-NIE-rnd-RC-RA-vs-nb-monitors}). 



\myitemit{Key finding:} \textit{The NIE with monitors of public services estimates the impact with an error within $\pm 10\%$ in most cases, and within $\pm 20\%$ in almost all cases.}

We present the distribution of the (absolute) error in the estimations of NIE with RC monitors in Fig.~\ref{fig:sims-impact-rc-vs-hijack-types-abs-error} (the case of NIE with RA monitors is similar%, see Appendix~\ref{appendix:naive-method}
). As can be seen, in more than 60\% of the cases for hijack Type-0 (red line, $y=0.6$), the error is lower than 10\% ($x=0.1$), while for Type-2 this holds for more than 80\% of the cases. Furthermore, in all cases, the error is almost always lower than $20\%$.


\begin{figure}
\centering
\subfigure[absolute error]{\includegraphics[width=0.49\linewidth]{./figures/fig_impact_RC_vs_hijackTypes_absError.eps}\label{fig:sims-impact-rc-vs-hijack-types-abs-error}}
\caption{CDF of the absolute error of NIE (i.e., $|\hat{I}_{NIE}-I|$) with all the RC monitors for hijacks of Type-0, 1, and 2.}
\label{fig:}
\end{figure}


\subsection{Towards Designing Impact Estimation Methods}
Below we discuss some practical aspects on the implementation of the NIE, which --in combination with the above findings-- lead our design for the hijack impact estimation methodology based on ping campaigns we propose in the following section.



% Based on the above findings and the insights stemming from them, we proceed to design a hijack impact estimator methodology, by focusing on both the achievable accuracy and practical aspects. 

% Below we discuss --for the different impact estimation approaches-- the main implementation and system design issues, as well as technological challenges and limitations. These aspects lead us to propose two methodologies and drive our design choices. The two methodologies, one based on ping campaigns (Section~\ref{sec:ping-estimator}) and one based on feed from RC monitors (Section~\ref{sec:ml-estimator}), are presented in detail and evaluated in the following sections.


\myitem{Random monitors vs. Public services:} Our results show that selecting monitors randomly (among all ASes in the Internet) results in significantly lower error (\pavlos{and very close to its lower bound for $M\ge 100$}). Thus, estimations using random monitors should be preferred when accuracy is the main goal. However, this approach can be implemented only through ping campaigns, since public services do not have monitors in all ASes. 

\myitem{Ping campaigns: challenges and limitations.} Measuring with pings whether a monitor is infected can have some challenges and limitations in practice. Pinging an IP address, does not necessarily mean that it will reply; in fact, a very small fraction of the addresses in the IP space respond to pings~\cite{pingable-ip-2013,heidemann2008census}. While there are lists of ``pingable'' IP addresses per AS~\cite{antlabhitlists}, they still not always respond to pings. If a monitor does not reply to a ping request, then we may falsely infer the monitor as infected, and thus overestimate the impact of the hijack. To overcome this challenge, in Section~\ref{sec:ping-estimator} we first study and quantify the effect of ping failures, and then design a methodology that can still be accurate, by carefully selecting the set and number of IPs per AS to ping.

Moreover, a limitation of the ping measurements approach is that it is not applicable in the case of man-in-the-middle (MitM) attacks%, where the traffic crosses the hijacker's network and is forwarded to the victim
, since all replies will end up to the victim, thus falsely denoting that the monitor is not infected\footnote{While there exist techniques that compare the RTT of a ping before and after a hijack to infer whether there is a MitM attack\pavlos{REFs: some hijack detection works}, these are mostly based on aggregate statistics (RTT among many pings), and are not expected to be accurate for \textit{every} ping measurement. This would lead to high failure probability, and thus inaccurate estimations.}. In this case, we could still use an approach based on control-plane information (e.g., BGP updates and traceroutes from public monitors).
\pavlos{needs better argumentation here}
 

% However, the ping campaign methodology is still not applicable in the case of MitM attacks; also, it requires active measurements which add a small extra overhead (e.g., deployment of a system to trigger and monitor the pings). Hence, as an alternative (and/or for completeness), we design a methodology based on control-plane \vkotronis{why not also data-plabe (RA)?} information from monitors of the public services. The public services methodology needs to overcome some challenges and limitations that have been indicated by our analysis (e.g., lower accuracy - Fig.~\ref{fig:RMSE-NIE-rnd-RC-RA-vs-nb-monitors}) and are discussed in more detail below.

